Space and Time Bounded Multiversion Garbage Collection

We present a general technique for garbage collecting old versions for multiversion concurrency control that simultaneously achieves good time and space complexity. Our technique takes only $O(1)$ time on average to reclaim each version and maintains only a constant factor more versions than needed (plus an additive term). It is designed for multiversion schemes using version lists, which are the most common. Our approach uses two components that are of independent interest. First, we define a novel range-tracking data structure which stores a set of old versions and efficiently finds those that are no longer needed. We provide a wait-free implementation in which all operations take amortized constant time. Second, we represent version lists using a new lock-free doubly-linked list algorithm that supports efficient (amortized constant time) removals given a pointer to any node in the list. These two components naturally fit together to solve the multiversion garbage collection problem--the range-tracker identifies which versions to remove and our list algorithm can then be used to remove them from their version lists. We apply our garbage collection technique to generate end-to-end time and space bounds for the multiversioning system of Wei et al. (PPoPP 2021).

==> application-old.tex <==
% !TEX root =  main.tex

\section{Application to Snapshottable Data Structures}
\label{sec:application}

\Eric{I find this section a bit confusingly organized.}
\Hao{we use both "multi-versioning" and "multiversioning" throughout the paper}
\Eric{We agreed to use multiversion}
\Yihan{We are also using both ``version list data structure'' and ``version-list'' data structure}
\Hao{There's some repetition in this paragraph with the related works, but I think it's a useful reminder of how ~\cite{WBBFRS21a} works.}
\Eric{See comment in related work about possibly merging with paragraphs from related work section}

In this section, we give a concrete example of how to apply our range-tracking object and version-list data structures for multiversion garbage collection.
Wei et al.~\cite{WBBFRS21a} described a technique for making concurrent data structures snapshottable using multiversioning.
As described in Section~\ref{sec:related}, they introduce a Camera object which is used to take snapshots of a set of VersionedCAS objects.
Multiversioning can be applied to a concurrent data structure implemented from CAS objects by replacing each CAS object with a VersionedCAS object, all associated with the same Camera object.
For a large class of concurrent data structures, arbitrary read-only operations can be supported by first taking a snapshot of all the VersionedCAS objects
\Eric{We should be avoid saying "take a snapshot of all the objects" because
a DISC reviewer may interpret this to mean "make a local copy of all objects" (as
reviewers of earlier incarnations of our PPOPP paper did) and consequently give up right here
because this approach sounds hopelessly impractical.  The more careful discussion of handles
in the related work section is better.}
using the Camera object and then running a sequential version of the operation on the snapshot.
\Yihan{Alternative way (maybe make it shorter?): For a large class of concurrent data structures, arbitrary read-only operations can be supported by first acquiring a handle from the Camera object, which can be used to access the corresponding versions of each VersionedCAS object at that time, and then running a sequential version of the operation on the snapshot, which ensures the query work on a snapshot of the data structure without making a deep copy.
}
A complication when using this approach is that reclaiming memory becomes more challenging.
In this section, we show how to use the techniques presented earlier in the paper to reclaim memory while maintaining good time and space bounds.
%The exact bounds we achieve are stated in Theorems~\ref{} and~\ref{}.
\Hao{mention somewhere that we only cover indirect VersionedCAS objects.}

We divide operations on
snapshottable data structures into \emph{snapshot queries},
which are query operations that run on a snapshot of the data structure,
and \emph{frontier operations},
which are operations inherited from the original non-snapshottable data structure.

\Eric{It would be really helpful in the following to distinguish vnodes and dnodes}
%We apply our technique as follows.
The original implementation of a VersionedCAS object stores a history of all of the object's
previous values in a singly-linked version list.  We instead use the
doubly-linked list from Section~\ref{sec:vlists} with the memory reclamation scheme from Section~\ref{sec:smr-list} to allow unneeded versions to be efficiently removed from the middle of the list and reclaimed.
We use a single range-tracking object \op{rt} to store nodes
that have been unlinked from the current version of the data structure, but might be still reachable from older snapshots.
Whenever a \op{vCAS} operation adds a new node to the head of a doubly linked list, we \op{deprecate} the previous head.
More specifically, if \C\ is appended after \B, then \op{rt.deprecate(B, B.timestamp, C.timestamp)} is called.
Next, we modify the \op{Camera.takeSnapshot} operation so that it announces the current value of the Camera object's timestamp field using \op{rt.announce(\&Camera.timestamp)} before attempting to increment this timestamp.
This announcement prevents nodes that are part of this snapshot from being returned by the \op{deprecate} operation.
Once a process is done using the snapshot, it calls \op{Camera.unreserve} to undo the announcement.
This means that once a version list node (\vnode{}) is returned by \op{deprecate}, it is not needed by any ongoing snapshot query, so we can \co{remove} it from the doubly-linked list.
In order to get good space bounds using Theorem~\ref{thm:step3-space}, we need to bound the number ($K$) of reference-counted pointers to \vnode{}s that are held outside of the version list algorithm.
We ensure that $K \in O(P)$ by having the range-tracking data structure store raw pointers to \vnode{}s rather than reference-counted ones.
Once a raw pointer is returned by the range-tracking data structure, it is safe to convert it back into a reference-counted pointer because \op{remove} has not been called on it, so the node it points to is guaranteed to not be freed.
%This means that after a \vnode{} is returned by \op{deprecate}, we have to first convert it into a reference-counted pointer before passing it
These changes are shown in blue in Figure~\ref{fig:vcas-alg-youla-gc}.
\Hao{This description may not be clear to someone who is not familiar with our PPoPP paper, but making it more clear would require more space.}

There are three types of objects in the snapshottable data structure: objects from the original data structure (\dnode{}s), version list nodes (\vnode{}s), and Descriptor objects.
\Eric{Move preceding sentence earlier}
The reclamation of \vnode{}s and Descriptors are handled by the reference-counting scheme introduced in Section~\ref{sec:smr-list}, as described in the previous paragraph.
A \dnode{} can be reclaimed when neither frontier nor snapshot operations need it any longer.
We assume that the basic data structure comes with a memory reclamation scheme, and this is used to determine if a \dnode{} is needed by any frontier operation.
We make no assumptions about the original memory reclamation scheme except that it calls \op{retire} on a node when it becomes unreachable from the roots of the data structure and \op{free} on a node when it is safe to collect.
Operations invoked after a node is retired cannot possibly reach the node, but operations
that were in progress when it was retired might
still access it.
Many existing memory reclamation schemes, including hazard-pointers~\cite{HL+05}, hazard-eras~\cite{RC17}, and epoch based collection~\cite{Fra04}, fit into this framework.
When the original data structure's memory reclamation scheme \op{free}s a node,
we know that it will not be needed by any frontier operation,
so we just need to track which \dnode s are needed by the snapshot queries.
This is done by tagging each \dnode{} with a birth and retire timestamp.
After a \dnode\ is allocated but before it is attached to the data structure,
its birth timestamp is set by reading the Camera
object's timestamp field and writing it into the appropriate field of the \dnode{}.
Similarly, a \dnode's retire timestamp is set when the original data structure's
memory reclamation scheme calls \op{retire} on the node.
A \dnode{} is not needed by any snapshot operation if there is no announced timestamp between
its birth timestamp (inclusive) and retire timestamp (exclusive).
We track this using the same \rangetracker{} data structure \op{rt} introduced earlier.
%We track this using the \rangetracker{} data structure from Section \ref{sec:identify}.
%The instance of the \rangetracker{} data structure for
%\dnode{}s is separate from the one for \vnode{}s, but they share the same announcement array.
Whenever the original data structure's memory
reclamation scheme \op{frees} a \dnode{} \op{N},
we instead call \op{rt.deprecate(N, N.birthTS, N.retireTS)}.
When a \dnode{} gets returned by a \op{deprecate},
we first call \op{remove} on the \vnode\ at the head of any
version lists pointed to by the \dnode{} and then free the \dnode{}.
The calls to \co{remove} is important because without it, the heads of the version
lists would never be collected. \dnode{}s returned by the range-tracking object are
safe to free because they are not needed by any frontier or snapshot operation.

We consider a \dnode{} to be \emph{necessary} if it is either not freed by the original data structure's memory reclamation scheme or if there exists an announced timestamp in between its birth (inclusive) and retire (exclusive) timestamp.
We say that a \vnode{} is \emph{necessary} if it is pointed to by a \dnode{} that has not yet been deprecated (i.e. freed by the original data structure's memory reclamation scheme) or if it has been deprecated but the interval it was assigned contains an announced timestamp.
Let $D_{max}$ and $V_{max}$ be the maximum number of necessary \dnode{}s and \vnode{}s throughout a history.

\Hao{provide some intuition / examples for the bounds below. Especially the time bounds.}
\Hao{We assume that all \dnode{}s take up $O(1)$ space (memory words).}

\begin{restatable}{theorem}{applicationSpace}
\label{thm:overall-space}
	The overall space usage of a memory-managed snapshottable data structure is $O(D_{max} + V_{max} + P^2 \log P + P^2 \log L)$, where $L$ is the number of successful \op{vCAS} operations.
\end{restatable}

%The following theorem assumes that snapshot queries visit each , which is possible to achieve via caching.
%
%For snapshot queries to be time efficient, it is important to avoid traversing the same version list multiple times.
%This can be avoided by caching the value read from each version list.


\begin{restatable}{theorem}{applicationTime}
\label{thm:overall-time}
	Snapshot queries take amortized expected time proportional to its sequential complexity plus the number of \op{vCAS} instructions concurrent with it.
	The amortized expected time complexity of frontier operations remains unchanged.
\end{restatable}



\Hao{TODO:
\begin{itemize}
	\item verify that all assumptions require by range-tracker and version-lists hold.
	\item intuitively state the space bounds for \vnode{}s and \dnode{}s (constant factor of necessary plus some additive term)
	\item briefly justify time and space bounds for \vnode{}s and \dnode{}s.
\end{itemize}
}


%This is actually a fairly complicated application of our techniques because adding multiversioning also makes the memory management of data structure nodes (\dnode{}s) more difficult.
%A node that could have been freed by the original non-snapshottable data structure might not be safe to free in the snapshottable data structure as these nodes could still be reachable by

%\Hao{This is actually a fairly complicated application because in addition to version list nodes, there are also data structure nodes that are reachable from old versions and need to be memory managed.} 

==> direct-vcas.tex <==

\section{Reclaiming Memory in Direct vCAS Algorithm}

Notes:
\begin{itemize}
	\item For the theory part of the paper, it's fine to avoid retiring the two tail nodes in each version list. But to maintain our memory bounds, we need to clear all the non-version list pointers in these nodes when they are returned by the interval tracker data structure. This might be a little difficult for the tail node because it gets added to the interval tracker multiple times. We can deal with a reference count in each node counting the number of version lists its in. There shouldn't be any races between decrementing to 0 and incrementing back to 1. We don't need this counter in the indirect case because each VNode is only in one version list.
	\item In the practical side of the paper, we will briefly describe how these two nodes can be retired. I wonder if this will make a big difference in practice.
	\item Tail nodes don't have back pointer so when you retire a tail node, you might have to add both the tail and the node that replaced it into the interval tracker data structure and prevent the replacing node from being removed until the tail is removed. Although you have to remember to clear all the pointers in the replacing node when you logically remove it.
\end{itemize}

% \input{version-list-alg-direct}

==> macros_backup.tex <==
% !TEX root =  main.tex

\def\draft{1}  % set to 1 for draft (include comments, color edits), 0 for clean final copy (omit comments, edits in black)
\if\draft 0
\newcommand{\mycomment}[3]{{\color{#2}{[\textbf{#1: #3}]}}}
\newcommand{\myedit}[2]{{\color{#1}{#2}}\normalcolor}
\newcommand{\rebuttaledit}[2]{{\color{#1}{#2}}\normalcolor}
\usepackage{showkeys}
\else
\newcommand{\mycomment}[3]{}
\newcommand{\rebuttaledit}[2]{#2}
\newcommand{\myedit}[2]{#2}
\fi



\newcommand{\Eric}[1]{\mycomment{Eric}{magenta}{#1}}
\newcommand{\Guy}[1]{\mycomment{Guy}{olive}{#1}}
\newcommand{\Hao}[1]{\mycomment{Hao}{brown}{#1}}
\newcommand{\Naama}[1]{\mycomment{Naama}{blue}{#1}}
\newcommand{\Yihan}[1]{\mycomment{Yihan}{purple}{#1}}
\newcommand{\Youla}[1]{\mycomment{Youla}{cyan}{#1}}

\newcommand{\er}[1]{\myedit{magenta}{#1}}
\newcommand{\y}[1]{\myedit{cyan}{#1}}
\newcommand{\hedit}[1]{\myedit{brown}{#1}}
\newcommand{\rebuttal}[1]{\rebuttaledit{cyan}{#1}}

\newcommand{\dnode}{DNode}
\newcommand{\vnode}{VNode}
\newcommand{\rcptr}{\texttt{rc\_ptr}}
\newcommand{\arcptr}{\texttt{arc\_ptr}}
\newcommand{\rangetracker}{range-tracking}

\newcommand{\downptr}{down-pointer}
\newcommand{\lrunreachable}{lr-unreachable}
\newcommand{\srcnode}{source-node}
\newcommand{\lrreachable}{lr-reachable}
\newcommand{\upptr}{up-pointer}

\newcommand{\future}[1]{} % used for comments about things to think about in the future (not current submission)


\newcommand{\hil}[1]{\color{blue}{#1}}

\newcommand{\myparagraph}[1]{\vspace{.03in}\noindent {\bf #1}} % NOTE:  LIPICS instructions specifically say not to do this!
%\newcommand{\myparagraph}[1]{\subparagraph*{#1}} 

\newcommand{\op}[1]{\co{#1}} % Use this for operation names
\newcommand{\unmarked}{\texttt{unmarked}}
\newcommand{\marked}{\texttt{marked}}
\newcommand{\finalized}{\texttt{finalized}}

\newcommand{\rmv}{\texttt{remove}}
\newcommand{\vread}{\texttt{vRead}}
\newcommand{\readver}{\texttt{readVersion}}
\newcommand{\vcas}{\texttt{vCAS}}

\newcommand{\retireInterval}{\op{deprecate}}
\newcommand{\Announce}{\op{announce}}
\newcommand{\Unannounce}{\op{unannounce}}
\newcommand{\NULL}{{\tt NULL}}

\newcommand{\RT}{{\sc RangeTracker}}

\newcommand{\snapshot}{camera}
\newcommand{\vCAS}{versioned CAS}

\newcommand{\announce}{{\tt Ann}}
\newcommand{\retired}{\co{LDPool}}
\newcommand{\qretired}{\co{QDPool}}
\newcommand{\free}{\op{Redundant}}
\newcommand{\Needed}{\op{Needed}}
\newcommand{\Redundant}{\op{Redundant}}
\newcommand{\queue}{{\tt Q}}
\newcommand{\Empty}{\mbox{$\bot$}}
\newcommand{\freed}{Free}

\newcommand{\merge}{\op{merge}}
\newcommand{\sortAnnouncements}{\op{sortAnnouncements}}
\newcommand{\sort}{\op{sort}}
\newcommand{\toArray}{\op{toArray}}
\newcommand{\intersect}{\op{intersect}}
\newcommand{\Split}{\op{split}}

\lstset{basicstyle=\scriptsize\ttfamily, tabsize=2, escapeinside={@}{@},
	columns=flexible, showstringspaces=false, frame=single, numberblanklines=false,
	numberstyle=\scriptsize, numbersep=3pt}
\lstset{literate={<|}{{$\langle$}}1  {|>}{{$\rangle$}}1}
\lstset{language=C++, morekeywords={CAS,and,or,in,each,commit,empty,new,job,taken,entry,GOTO,bool,extends}}
%\lstset{xleftmargin=5.0ex, numbers=left}
%\lstset{caption={\texttt{tuple} and \collect{} algorithms},captionpos=b,label={alg:collect}}
\makeatletter
\lst@Key{countblanklines}{true}[t]%
{\lstKV@SetIf{#1}\lst@ifcountblanklines}

\def\ContinueLineNumber{\lstset{firstnumber=last}}
\def\StartLineAt#1{\lstset{firstnumber=#1}}

\lst@AddToHook{OnEmptyLine}{%
	\lst@ifnumberblanklines\else%
	\lst@ifcountblanklines\else%
	\advance\c@lstnumber-\@ne\relax%
	\fi%
	\fi}
\makeatother


\newcommand{\here}[1]{{\bf [[[ #1 ]]]}}
\newcommand{\HERE}[1]{{\bf [[[ #1 ]]]}}

\newcommand{\ignore}[1]{}

\newtheorem{theorem}{Theorem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{claim*}{Claim}

\renewcommand\qedsymbol{\textcolor{lipicsGray}{\ensuremath{\blacktriangleleft}}}
\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\labelsep
        \color{lipicsGray}\sffamily\bfseries
    #1\@addpunct{.}]\ignorespaces
}{%
  \popQED\endtrivlist%\@endpefalse
}
\newcommand{\claimqedhere}{\renewcommand\qedsymbol{\textcolor{lipicsGray}{\ensuremath{\vartriangleleft}}}%
\qedhere%
\renewcommand\qedsymbol{\textcolor{lipicsGray}{\ensuremath{\blacktriangleleft}}}}
\newenvironment{claimproof}[1][\proofname]{
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\labelsep
        \color{lipicsGray}\sffamily
    #1\@addpunct{.}]\ignorespaces
}{%
  \renewcommand\qedsymbol{\textcolor{lipicsGray}{\ensuremath{\vartriangleleft}}}
  \popQED\endtrivlist%\@endpefalse
  \renewcommand\qedsymbol{\textcolor{lipicsGray}{\ensuremath{\blacktriangleleft}}}
}

\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{invariant}[theorem]{Invariant}

\newcommand{\MRS}{MRS}

\newcommand{\co}[1]{\mbox{\tt #1}}
\newcommand{\A}{\co{A}}
\newcommand{\B}{\co{B}}
\newcommand{\C}{\co{C}}
\newcommand{\D}{\co{D}}
\newcommand{\E}{\co{E}}
\newcommand{\U}{\co{U}}
\newcommand{\V}{\co{V}}
\newcommand{\W}{\co{W}}
\newcommand{\X}{\co{X}}
\newcommand{\Y}{\co{Y}}
\newcommand{\Z}{\co{Z}}
\newcommand{\ts}{\co{ts}}

\newcommand{\sul}{\co{spliceUnmarkedLeft}}
\newcommand{\sur}{\co{spliceUnmarkedRight}}
\newcommand{\spl}{\co{splice}}
\newcommand{\frozen}{\co{frozen}}


\theoremstyle{definition}
\newtheorem{assumption}[theorem]{Assumption}



==> memory-reclamation-pseudo-code.tex <==
\begin{figure*}[!thp]\small
  %\vspace{-.1in}
  \hspace{-10mm}
  \begin{minipage}[t]{.55\textwidth}
    \begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none]
class Node {
  arc_ptr<Node> left, right; // initially null
  enum status {unmarked,marked,finalized};
  // initially unmarked
  int counter; // used to define priority
  int priority; // defines implicit tree
  int ts; // timestamp
  arc_ptr<Descriptor> leftDesc, rightDesc;  // initially null
  @\hil{int refCount;}@ };

class Descriptor {
  arc_ptr<Node> A, B, C;
  @\hil{int refCount;}@ };
rc_ptr<Descriptor> frozen = new Descriptor();

class VersionList {
  arc_ptr<Node> Head;
  // public member functions:
  rc_ptr<Node> getHead() {return Head;}
  rc_ptr<Node> find(rc_ptr<Node> start, int ts) {
    rc_ptr<Node> current = start;
    while(current->ts > ts) {
      @\hil{rc\_ptr<Node> next = current->left;}@
      @\hil{if(next == $\top$) next = current->right;}@
      @\hil{current = next;}@ }
    return current; } };

  bool tryAppend(rc_ptr<Node> B, rc_ptr<Node> C) {
    if(B != null) {
      C->counter = B->counter+1;
      rc_ptr<Node> A = B->left;             @\label{mr-read-left-gc}@
      @\hil{if(A == $\top$) return false;}@   @\label{check-top-gc}@
      if(A != null) A->right.CAS(null, B); @\label{mr-cas1-gc}@
    } else C->counter = 2;
    C->priority = p(C->counter);          @\label{set-priority-gc}@
    C->left = B;                  @\label{set-left-gc}@
    if(Head.CAS(B, C)) {              @\label{head-cas-gc}@
      if(B != null) B->right.CAS(null, C); @\label{mr-cas2-gc}@
      return true;
    } else return false; }

  // public static functions:
  void remove(rc_ptr<Node> B) {
    // B cannot be null
    B->status = marked;         @\label{mark-gc}@
    for F in [leftDesc, rightDesc] {
      repeat twice {          @\label{repeat-twice-gc}@
        rc_ptr<Descriptor> desc = B->F;   @\label{read-desc1-gc}@
        help(desc); @\label{remove-help-gc}@
        B->F.CAS(desc, frozen); @\label{freeze-desc-gc}@ } }
    removeRec(B); }           @\label{call-rr1-gc}@

  // private helper functions:
  bool validAndFrozen(rc_ptr<Node> X) {
    // rightDesc is frozen second
    return X != null && X->rightDesc == frozen; }

  void help(rc_ptr<Descriptor> desc) {
    if(desc != null && desc != frozen)      @\label{test-frozen-gc}@
      splice(desc->A, desc->B, desc->C); }  @\label{help-splice-gc}@

  int p(int c) {
    k = floor(log@$_2$@(c));
    if(c == 2^k) return k;
    else return 2k + 1 - lowestSetBit(c); }
  \end{lstlisting}
\end{minipage}\hspace{.3in}
\begin{minipage}[t]{.65\textwidth}%xleftmargin=5.0ex,
  \StartLineAt{59}
  \begin{lstlisting}[linewidth=.99\textwidth, numbers=left, frame=none]
// private helper functions continued:
void removeRec(rc_ptr<Node> B) {
  // B cannot be null
  rc_ptr<Node> A = B->left;             @\label{read-left-gc}@
  rc_ptr<Node> C = B->right;              @\label{read-right-gc}@
  if(B->status == finalized) return;          @\label{test-unfinalized-gc}@
  int a, b, c;
  if(A != null) a = A->priority;
  else a = 0;
  if(C != null) c = C->priority;
  else c = 0;
  b = B->priority;
  if(a < b > c) { @\label{test-priority-gc}@
    if(splice(A, B, C)) {               @\label{call-splice-gc}@
      if(validAndFrozen(A)) {
        if(validAndFrozen(C) && c > a) removeRec(C);    @\label{recurse1-gc}@
        else removeRec(A); }  @\label{recurse2-gc}@
      else if(validAndFrozen(C)) {
        if(validAndFrozen(A) && a > c) removeRec(A);    @\label{recurse3-gc}@
        else removeRec(C); } }  } @\label{recurse4-gc}@
  else if(a > b > c) {
    if(spliceUnmarkedLeft(A, B, C) && @\label{call-sul-gc}@
    validAndFrozen(C)) {
      removeRec(C); } }       @\label{recurse5-gc}@
  else if(a < b < c) {
    if(spliceUnmarkedRight(A, B, C) && @\label{call-sur-gc}@
    validAndFrozen(A)) {
      removeRec(A); } } } }     @\label{recurse6-gc}@

bool splice(rc_ptr<Node> A, rc_ptr<Node> B, rc_ptr<Node> C) {
  // B cannot be null
  if(A != null && A->right != B) return false;              @\label{test-right-gc}@
  bool result = CAS(&(B->status), marked, finalized);    @\label{finalize-cas}@
  if(C != null) C->left.CAS(B, A);                    @\label{left-cas-gc}@
  if(A != null) A->right.CAS(B, C);                   @\label{right-cas-gc}@
  @\hil{if(A != null \&\& A->priority > B->priority)}@
      @\hil{B->left = $\top$;}@     @\label{clear-left-gc}@
  @\hil{if(C != null \&\& C->priority > B->priority)}@
      @\hil{B->right = $\top$;}@    @\label{clear-right-gc}@
  return result; }

bool spliceUnmarkedLeft(rc_ptr<Node> A, rc_ptr<Node> B, rc_ptr<Node> C) {
  // A, B cannot be null
  rc_ptr<Descriptor> oldDesc = A->rightDesc;        @\label{read-desc2-gc}@
  if(A->status != unmarked) return false;
  help(oldDesc);                @\label{sul-help-old-gc}@
  if(A->right != B) return false;        @\label{sul-test-right-gc}@
  rc_ptr<Descriptor> newDesc = new Descriptor(A, B, C); @\label{create-right-desc-gc}@
  if(A->rightDesc.CAS(oldDesc, newDesc)) {   @\label{store-right-desc-gc}@
    // oldDesc != frozen
    help(newDesc);                 @\label{sul-help-new-gc}@
    return true;
  } else return false; }

bool spliceUnmarkedRight(rc_ptr<Node> A, rc_ptr<Node> B, rc_ptr<Node> C) {
  // B, C cannot be null
  rc_ptr<Descriptor> oldDesc = C->leftDesc;     @\label{read-desc3-gc}@
  if(C->status != unmarked) return false;     @\label{sur-test-marked-gc}@
  help(oldDesc);                @\label{sur-help-old-gc}@
  if(C->left != B || (A != null && A->right != B)) return false;        @\label{sur-test-???-gc}@
  rc_ptr<Descriptor> newDesc = new Descriptor(A, B, C); @\label{create-left-desc-gc}@
  if(C->leftDesc.CAS(oldDesc, newDesc)) {  @\label{store-left-desc-gc}@
    // oldDesc != frozen
    help(newDesc);                 @\label{sur-help-new-gc}@
    return true;
  } else return false; } };
  \end{lstlisting}
\end{minipage}
\vspace{-.1in}
\caption{Implementation of version lists with memory management.
\Eric{Just give new versions of splice and tryAppend, and mention in text that refcounts are added to Node and Descriptor}
\Eric{Right now, this figure is causing trouble with multiply-defined labels}
}
\Hao{I changed the labels so that they are unique}
\label{fig:list-alg-full-gc}
\end{figure*}

==> overview.tex <==
% !TEX root =  main.tex

\section{Introduction}

The design of concurrent data structures is a central problem in shared-memory distributed computing,
and has been a subject of active research in recent decades.
Most of this work has focused on providing operations that read or modify localized portions
of the data structure.  For example, a data structure representing a set might provide
operations to insert and delete elements, and to search for a given element.
There are many applications, however, where query operations require a consistent view
of a larger part of the data structure. For example, a range query on an ordered set
returns all elements that are between two given values.
\Youla{What do we mean with "localized portions" of the data structure?}

Supporting more complex query operations in a lock-free manner is the subject of much recent work,
although it has primarily focused on specific queries for specific data structures.
\y{For example, there have been several implementations of linearizable range queries
on a variety of data structures \cite{AB18,BA12,Cha17,FPR19}.
Recently, Wei et al.~\cite{WBBFRS21a} gave a general technique for adding wait-free query operations
to a lock-free data structure based on CAS instructions.
Their approach is based on multiversion concurrency control \cite{Reed78}.
Each CAS object is replaced by a {\it versioned CAS} object that stores a linked list
of all values that have ever been stored in the object, with associated timestamps.
A query operation can navigate these lists to read the version of the data structure that was
current at a particular timestamp.
%This approach could lead to significant memory overhead, but Wei et al.\ used
%epoch-based memory reclamation \cite{Fra04} to collect old versions that were no longer needed.
%Although this approach worked well in experiments, there was no bound on the amount of memory required.
%In this paper, we describe a memory reclamation scheme that can more precisely
%identify old versions to be collected, so that we can give a good overall bound on the memory
%usage of the multiversioning scheme.
%Because multiversioning is widely applicable, we believe
% aspects of this paper will be useful in other contexts.
%\Naama{The intro up to here sounds much more narrow than the abstract and title.}

The design of general query operations for lock-free data structures
typically %requires significant effort and
introduces new issues for garbage collection,
which is already a challenging problem in the context of lock-free data structures.
For instance, the use of multi-versioning} %, as is the case with the approach in~\cite{WBBFRS21a}, }
could lead to significant memory \y{overhead. Wei {\em et al.}~\cite{WBBFRS21a}\ used
epoch-based memory reclamation \cite{Fra04} to collect old versions that were no longer needed in~\cite{WBBFRS21a}.}
%Although this approach worked well in experiments, there was no bound on the amount of memory
%required.
\y{However, this approach did not provide any bound on the amount of memory
required.}

\y{In this paper, we describe a memory reclamation scheme that can more precisely
identify old versions to be collected. We apply this scheme on top of the
multiversioning scheme provided in~\cite{WBBFRS21a} to get a good overall bound
on its memory usage. % of the multiversioning scheme in~\cite{WBBFRS21a}.
Doing so turned out to be a complex task requiring to cope with complications
in three different dimensions: 1) identify nodes in the version lists
representing old versions that can be collected, 2) splice nodes representing obsolete versions out of their version lists,
and 3) actually free memory when it is no longer needed.
Our scheme provides solutions to all these problems.
Because multiversioning is widely applicable, we believe
that our results will be useful in other contexts.}
\Youla{What about time complexity? I think we need to say something here
as it was also not trivial to come up with the time bound. }
\Eric{Reduce repetition between this paragraph and the following ones}

\y{Specifically, we divide the memory management problem into three tasks.
The first focuses on identifying the nodes in the version lists representing obsolete versions that can be collected.
Assuming a kind of generic multi-versioning scheme (e.g., that in~\cite{WBBFRS21a}),
we were able to abstract this problem by specifying a {\it range-tracking object} that is used to
identify obsolete versions in the version lists.
The range-tracking object supports a \co{\retireInterval} operation that is
applied to a version \co{o} when it is superseded by another
(i.e., when a CAS instruction updates a value).
This operation returns a list of deprecated objects
that have become obsolete and are safe to be disconnected and collected.
To come up with an efficient implementation of the range-tracking object,
1) we have each process announcing the timestamp value it is using for a query operation
and we employ a mechanism from~\cite{} to make a process' announcement phase
wait-free,
and 2) we assign to each node in the version list an interval of timestamp values representing the
range of time during which that version was the current value of a CAS object.
Any old (non-current) version whose interval does not intersect the set of announced timestamps is obsolete.
}
We provide a novel implementation of a range-tracking object
for which  the
number of steps per \retireInterval\ is $O(1)$.
We also bound the number of objects on which \retireInterval\ has been called, but have not
yet been returned as obsolete.



\y{The second task copes with splicing} nodes representing obsolete versions out of their version lists.
To do this with the desired efficiency, we provide a new implementation of a lock-free
doubly-linked list. It permits new versions to be appended (only) at one end of the list,
but elements can be deleted from anywhere in the list.
\y{Nodes are first logically deleted by marking them and then they are physically deleted from the list.
Splicing a node from a doubly-linked list is a quite complicated task, as it requires to
ensure that two adjacent nodes cannot be spliced concurrently.
To achieve this, we assign priorities to version nodes,
and use ideas from tree contraction~\cite{} to utilize a priority tree
according to which we determine in which order the nodes should be spliced.
Specifically, we splice only nodes whose descendants in the
priority tree are all already spliced out of the list. This ensures that
a node is spliced out of the list only if its priority is greater than
its neighbours, and therefore the removal of two consecutive list nodes
is prevented. However, this mechanism alone was not enough,
as one unmarked node could block its ancestors in the priority tree from
being spliced out of the list, which could jeopardize the bounds we would like to achieve.
To address this, we came up with a novel and fairly intricate helping
mechanism to ensure that nodes are indeed physically removed from the list to achieve
our desired complexity bounds.
}
The amortized number of steps performed by deletions is $O(1)$.
An attempt to append a node takes $O(1)$ steps in the worst case,
but it may fail if another concurrent append succeeds.
Crucially, the number of nodes that remain reachable is at most double the number of nodes
that should be in the list, plus $O(P\log L)$, where $L$ is the total number of nodes
successfully appended to the list. \Naama{Might be good to compare to previous work on doubly-linked lists.}
\Youla{I have expanded the discussion above a little bit more, as I consider this to be the most
difficult/important part of the paper and possibly also the part that contributes more in terms of novelty.}


\y{The third task is to} actually free memory when it is no longer needed.  The data structure that supports queries
includes objects that are part of the original data structure ({\it \dnode s}) and
nodes used to represent the version lists ({\it \vnode s}) in order to add support for queries.
We assume that the original data structure is equipped with a memory management scheme,
that frees \dnode s when they are no longer part of the data structure.
\y{Such a scheme is not sufficient though}
%must be modified
because those \dnode s might still be part of old versions
of the data structure required by queries. \Hao{mention that we just need to put a wrapper, without having to know anything about how the scheme works. Modifying the scheme sounds like a lot of work, so we should make this sound easier.} \Youla{I have made small changes to address Hao's comment.}
We use the range-tracking object described above a second time to manage \dnode s.
We use a reference-counting scheme to manage \vnode s. \y{We were able to implement these enhancements
using wrappers, without having to know how the original memory management scheme works.}


\Eric{State overall bounds achieved}

\y{We provide detailed formal proofs for all three parts. Due to lack of space,
they appear in the appendix.}

\ignore{
\Eric{Might be useful to have a diagram in the overview that shows how the various pieces of pseudocode scattered through the paper relate to one another (i.e., which Figures invoke procedures in other Figures)}
}

\ignore{
\section{Overview}

Step 1 involves identifying nodes which are safe to remove from the version lists. Step 2 describes how to unlink them, and Step 3 describes how to free the unlinked nodes.


\subsection{Step 1}

For Step 1, we define a \emph{range tracker} data structure with 3 operations. Their sequential specifications are provided below.

% TODO: this interface doesn't work well with HE because they have their own way of doing announcements.

\begin{itemize}
	\item \Announce(int* \co{ptr}): Atomically reads and announces the integer pointed to by \op{ptr}. Returns the value read as well as an \op{Announcement} object.
	\item \Unannounce(Announcement \co{$\alpha$}): Clears the announcement \co{$\alpha$}.
	This can be performed on a thread different from the one that created \op{a}.
	\item \retireInterval(T \co{t}, int \co{low}, int \co{high}): Retires an object $t$ and associates it with the interval [\op{low}, \op{high}).
	This operations also returns a list of objects of type \op{T} such that for each object $t$ in the list, (1) $t$ has been previously retired, but not returned, and (2) $t$'s associated interval is not intersected by any currently active announcements.
	An object may be retired multiple times (we need this for the direct vCAS algorithm) and an empty list may be returned.
%	\item \op{ejectInterval()}: Returns a node that has been retired, but not previously ejected, and who's associated interval is not intersected by any currently active announcements. If there's no such node, then null is returned instead.
\end{itemize}


Our implementation of the interval tracker data structure makes the following assumptions (which are satisfied by our applications):

\begin{itemize}
	\item Every time a process performs \retireInterval, the value it passes to \op{high} is monotonically increasing. This allows us to get \retireInterval\ down to amortized constant time.
	\item Whenever an integer is announced, it is higher than everything that was previously announced or passed as the \op{high} argument to any \op{retire}.
	% comes after the previously inserted intervals [TODO: reword to be more precise].
	\item Each process must alternate \op{announce} and \op{unannounce} calls, starting with \op{announce}. \Naama{should also say it has to be on the same index.}
\end{itemize}

\subsection{Step 3: freeing nodes}

\subsection{Step 2}

For Step 2, we implement a concurrent list data structure that supports the following operations: \op{append}, \op{getHead}, \op{find}, \op{remove}. Their sequential specifications are given below:

[TODO: Bulleted list of related work. Bulleted list for step 3. Proof of space bounds. Shared queue for step 1.]

[TODO: rename list to version list]

\begin{itemize}
	\item \op{constructor}: The list is initially empty with head pointing to null.
	\item \op{tryAppend(ListNode* old, ListNode* new)}: Adds \op{new} to the head of the list and returns true if the current head is \op{old}. Otherwise returns false. Assumes \op{new} is not null.
	\item \op{getHead()}: Returns a pointer to the \op{ListNode} at the head of the list (or null).
	\item \op{find(Predicate p)}: Returns a pointer to the first \op{ListNode} (starting from head) that satisfies \op{p} (or null if one does not exist). \footnote{Instead of \op{find}, we can support a \op{getNext} operation instead, but then we would have to define what it means to read the next pointer of a node that has already been removed. This also potentially lets us abstract out Step 3 in a nicer way.}
	\footnote{The \op{find} operation takes in a predicate instead of a timestamp because the list interface does not assume that each node has a timestamp field. We could add operations for getting and setting timestamps, but I'm not sure if it would simplify anything.}
	\item \op{remove(ListNode* n)}: Given a previously appended \op{ListNode}, removes it from the list. [TODO: put into algorithm environment.]
\end{itemize}

Our implementation of this list data structure makes the following assumptions (which are satisfied by our applications):

\begin{itemize}
	\item \op{remove} cannot be invoked on a node until a newer node is completely appended. This is important because back pointers are updated after the linearization point of \op{tryAppend}.
	\item For each \op{find} operation, first node in the list satisfying predicate \op{p} is the same for the duration of the operation.
	This means that we can linearize \op{remove} operations at the marking step (important because a remove might return before the node gets spliced out) and in the \op{find}, we can return a node without checking if it is marked.
	This also means we don't need to worry about newly appended nodes satisfying the predicate, so we can implement \op{find} by simply traversing the list and returning the first node satisfying the predicate that we see.
\end{itemize}
}


% TODO: figure out how to solve the problem previously solved by invalidNextv

%Direct vCAS algorithm:
%
%\begin{itemize}
%	\item The first call to \op{tryAppend} should not change any right pointers. Removing this node should also not change any right pointers. More generally, the right point of the initial node should not change. I guess the initial node does not need a left or right pointer because it will never be removed and no find operation will traverse past it. Maybe another condition is that the initial node satisfies the predicate of any find on this list. We should be able to unlink the initial node eventually right? In that case, we might want to say that there exists a node in the list satisfying the precondition. But that disallows null.
%	\item Maybe we want to add a special function for retiring an initial value. Alternatively, you can just leave the initial valuArrayes in there forever.
%	\item Maybe we want to have a separate linked list algorithms for direct and indirect vCAS. The algorithm for direct vCAS can create its own list nodes maybe. But this would disallow us from changing its timestamps.
%	\item Every node should have a special marker indicating whether or not it is the first node to be appended.
%	\item Maybe we should replace left and right with prev and next.
%\end{itemize}
%
%\begin{figure*}
%	\begin{minipage}[t]{.46\textwidth}
%		\begin{lstlisting}[linewidth=.99\columnwidth, numbers=left, frame=none]
%class Node extends ListNode {
%	/* other fields of the Node class */
%	int ts; };        // initially TBD
%class DirectVersionedCAS {
%	List<Node> list; Camera* C;
%	DirectVersionedCAS(Node* n, Camera* c) {
%		C = c;
%		// n could already belong to another list
%		// double check this is ok
%		list = List<Node>(n); // list constructor
%		initTS(n); }
%	void initTS(Node* n) {
%		if(n != NULL && n->ts == TBD) {
%			int curTS = C->timestamp;
%			CAS(&(n->ts), TBD, curTS); } }
%	Node* vRead() {
%		Node* head = list.getHead();
%		initTS(head);  @\label{line:getptr1}@
%		return head; }
%			\end{lstlisting}
%		\end{minipage}\hspace{.3in}
%		\begin{minipage}[t]{.46\textwidth}
%			\StartLineAt{19}%xleftmargin=5.0ex,
%			\begin{lstlisting}[linewidth=.99\textwidth, numbers=left,frame=none]
%	Node* readVersion(int ts) {
%		Node* node = Head; @\label{line:getptr2}@
%		initTS(node);
%		while(node != NULL && node->ts > ts)
%		node = node->nextv;
%		return node; }
%	bool vCAS(Node* oldV, Node* newV) {
%		Node* head = list.getHead();
%		initTS(head);
%		if(list.tryAppend(head, newV)) {  @\label{line:direct-append}@
%			initTS(newV); @\label{line:setts}@
%			return true; }
%		else {
%			initTS(Head);
%			return false; } } };
%		\end{lstlisting}
%	\end{minipage}
%	\vspace{-.1in}
%	\caption{Direct \vCAS{} implementation using the previously defined interval tracker and list data structures. I got rid of two if statements from vCAS because oldV can't be equal to newV in a successful vCAS, and if head != oldV, then this will be caught by the following CAS.
%		% \Eric{Line 9,26 assume Head is a simple pointer.  Line 17,20
%		%   assumes Head may be a marked pointer.  Can this be made more
%		%   consistent? }  \Guy{I suggest dropping all future
%		%   optimizations (i.e., getPtr and the CAS on line 30) from this
%		%   code.   We can then describe the diff, possibly even
%		%   including the modified lines.}
%	}
%	\label{fig:vcas-direct-alg}
%\end{figure*}

%\subsection{Step 3}




==> proof-list.tex <==
% !TEX root =  main.tex

\newpage

\section{Correctness of list maintenance}

\newcommand{\co}[1]{\mbox{\tt #1}}
\newcommand{\A}{\co{A}}
\newcommand{\B}{\co{B}}
\newcommand{\C}{\co{C}}
\newcommand{\D}{\co{D}}
\newcommand{\E}{\co{E}}
\newcommand{\U}{\co{U}}
\newcommand{\V}{\co{V}}
\newcommand{\W}{\co{W}}
\newcommand{\X}{\co{X}}
\newcommand{\Y}{\co{Y}}
\newcommand{\Z}{\co{Z}}

\begin{figure*}[!th]\small
	%\vspace{-.1in}
	\begin{minipage}[t]{.49\textwidth}
		\begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none]
// Worst-case time: O(log L) 
// where L is measured at the
// start of the operation
// Amortized time: O(1)

class Node {
	Node* left, right; // initially null
	enum status; // initially unmarked
	int priority; // defines implicit tree
};

void remove(Node* B) {
	B->status = marked;
	remove-rec(B); }

void remove-rec(Node* B) {
	Node* A = B->left;							@\label{read-left}@
	Node* C = B->right;							@\label{read-right}@
	bool recurse = false;
	if(A->priority > B->priority < C->priority) @\label{test-priority}@
		recurse = splice(A, B, C)               @\label{call-splice}@
	if(recurse) {
		if only one of {A, B} is marked,
		then call remove-rec() on whichever
		one is marked.
		If both are marked, then call
		remove-rec() on whichever one has
		smaller number. 
	} 
}

bool splice(Node* A, Node* B, Node* C) {
	Node* D = C->left;		   @\label{help-left-read}@
	if(D->left == B) 		   @\label{help-left-test}@
		CAS(&(C->left, D, B))  @\label{help-left-cas}@
	D = A->right;			   @\label{help-right-read}@
	if(D->right == B)          @\label{help-right-test}@
		CAS(&(A->right, D, B)) @\label{help-right-cas}@
	if (!CAS(&(B->status), marked, finalized)) @\label{finalize-cas}@
		return false;
	CAS(&(A->right), B, C);  @\label{right-cas}@
	CAS(&(C->left), B, A);   @\label{left-cas}@
	return true; }

bool tryAppend(Node* A, Node* B) {
	// Try to append node B after node A; succeeds if A is the last element of list
	// Return value says whether it was successful
	B->status = unmarked;
	B->counter = A->counter+1;
	B->priority = lowestSetBit(B.counter);
	B->left = A;                      @\label{set-left}@
	return CAS(&(A->right), null, B); @\label{append-cas}@
}
\end{lstlisting}
\end{minipage}
\vspace{-.1in}
\caption{Implementation of list operations
    \Eric{need a precondition of tryAppend that B is a new node.  Could we actually move the creation of B inside this routine?}
}
\label{fig:list-alg-simplified}
\end{figure*}

Consider the algorithm in Figure \ref{fig:list-alg-simplified}.
We say a node is {\it active} if it has been successfully appended to the list.
More precisely, a node becomes active when a pointer to it is stored by line \ref{append-cas} and it remains active forever after that.

Fix an execution.  We define two orderings on all the nodes that become active during the execution:
if \X\ and \Y\ are pointers to nodes, we write
$\X <_p \Y$ if $\co{X->priority} < \co{Y->priority}$ and $\X <_c \Y$ if $\co{X->counter} < \co{Y->counter}$.
The \co{counter} and \co{priority} fields of an active node never change, so this ordering is fixed.

We use the notation $\X \rightarrow \Y$ to mean $\co{X->right} = \Y$ and $\X \leftarrow \Y$ to mean $\co{Y->left} = \X$ and $\X \leftrightarrow\Y$ to mean $\X\leftarrow \Y$ and $\X\rightarrow \Y$.

\Eric{We'll probably need to say something about why the last node cannot be spliced to ensure that no two nodes get the same counter value, so that $<_c$ defines a total order on active nodes.  Maybe we just need a precondition on remove (for example, that the node's right pointer is non-null) to ensure this.}

\Eric{I'm abusing notation a little to use \X\ both for a node and a pointer to the node.}

\begin{lemma}
\label{order}
Let \X\ be any node.\\
When \co{X.right} is first set to a non-null value \Y, $\X <_c \Y$.  \\
Whenever the value of \co{X.right} changes from \Y\ to \Z, $\X <_c \Y <_c \Z$.\\
Similarly, when \co{X.left} is initialized to the value \W, $\W <_c \X$.  \\
Whenever the value of \co{X.left} changes from \W\ to \U, $\U <_c \W <_c \X$.\\
\end{lemma}
\begin{proof}
\co{X->right} is first set to a non-null value \Y\ at line \ref{append-cas} of \co{tryAppend}. 
$\X <_c \Y$ since $\co{Y->counter} = \co{X->counter} + 1$.
Similarly, \co{X->left} is first set at line \ref{set-left} of tryAppend, and again $\X <_c \Y$.

Consider any update to a right pointer.  Assume the claim holds in the prefix of the execution prior to this update.
\co{X->right} can subsequently be modified at line \ref{help-right-cas} or \ref{right-cas}.
If \co{X->right} is changed from \Y\ to \Z\ at line \ref{help-right-cas}, 
then the preceding test implies that $\Y \rightarrow \Z$, 
so by the induction hypothesis, $\Y <_c \Z$.
If \co{X->right} is changed from \Y\ to \Z\ at line \ref{right-cas} of a \co{splice(X,Y,Z)} then,
prior to calling \co{splice} at line \ref{call-splice}, \Z\ was read from \co{Y->right}.  
Thus, by the induction hypothesis, $\Y <_c \Z$.

The proof that updates to \co{X->left} satisfy the lemma is symmetric to the proof for right pointers.
\end{proof}

As a corollary of Lemma \ref{order} there is no ABA problem on \co{left} or \co{right} pointers of nodes.

\Eric{The following lemmas are trivial for the simplified algorithm without spliceUnmarkedLeft and spliceUnmarkedRight.  But I'm trying to extract from the proof properties we need to prove about how splice is called so that when we generalize to include spliceUnmarkedLeft/Right, we will just have to fix these lemmas.}

\begin{lemma}
\label{no-overlap}
There cannot be a call to \co{splice(W,X,Y)} and \co{splice(X,Y,Z)} in the same execution.
\end{lemma}
\begin{proof}
Suppose the claim is false.  Before \co{splice(W,X,Y)} is called on line \ref{call-splice}, the test on line \ref{test-priority} ensures that $\X <_p \Y$.  Similarly if \co{splice(X,Y,Z)} is called,
then $\X >_p \Y$.  A contradiction.
\end{proof}

\begin{lemma}
\label{splice-precond}
If \co{splice(A,B,C)} is called, there is some time prior to the call when $\A\leftarrow \B$ and another time prior to the call when $\B\rightarrow \C$.
\end{lemma}
\begin{proof}
Before \co{splice(A,B,C)} is called on line \ref{call-splice}, we have $\A\leftarrow \B$ at line \ref{read-left} and $\B\rightarrow\C$ at line \ref{read-right}.
\end{proof}

\Eric{following two lemmas should probably be folded together}

\begin{lemma}
\label{remove-safe}
If a node \Y\ is finalized, some process has called \co{remove(Y)}.
\end{lemma}
\begin{proof}
Node \Y\ can only be finalized inside a call to \co{splice(X,Y,Z)} at line \ref{call-splice} of \co{remove-rec(Y)}.
If the call to \co{remove-rec(Y)} was from \co{remove(Y)}, then the claim is true.
Otherwise the call to \co{remove-rec(Y)} was done recursively inside \co{remove-rec}.  
Before making this recursive call, \Y\ was observed to be marked.
\Y\ could only be marked by a call to \co{remove(Y)}.
\end{proof}

\begin{lemma}
\label{splice-marked}
Before \co{splice(A,B,C)} is called, \B\ is marked.
\end{lemma}
\begin{proof}
The call to \co{splice(A,B,C)} is made on line \ref{call-splice} of \co{remove-rec(B)}.
Before calling \co{remove-rec(B)} from the \co{remove(B)} routine, \B\ is marked.
Before calling \co{remove-rec(B)} recursively from \co{remove-rec}, \B\ must also be marked.
\end{proof}

\Eric{Remark:  Could actually do lines \ref{right-cas} and \ref{left-cas} in parallel without affecting the following proof; the order of those two steps is irrelevant.  Similarly for helping you could do lines \ref{help-left-read}--\ref{help-left-cas} and lines \ref{help-right-read}--\ref{help-right-cas} in parallel}

\Eric{Remark:  I just noticed that lines \ref{help-right-read} to \ref{help-right-cas} may be unnecessary, since the right pointer is always fixed before the left pointer, so the right pointer can never be inconsistent.  
Moreover, one case of claim \ref{well-formed} of the invariant can be eliminated.
In fact, we may want to swap line \ref{right-cas} and \ref{left-cas}, so that the left pointer is updated first and then the right pointer, and then remove lines \ref{help-left-read} to \ref{help-left-cas}.
The swap has the advantage of making sure left pointers are shortcutted first, making finds a tiny bit more efficient.
Unfortunately this breaks the symmetry of the algorithm so the proof may need to treat the currently symmetric cases slightly differently, but I think it should still be easy to write.

Hao also mentioned that the finalize-cas may be unnecessary; processes could instead return false if the first pointer cas failed.  This would require an overhaul of the proof:  a node would be deemed to be logically finalized when the left pointer to it is modified to skip past it.
}

\begin{lemma}
\label{rightmost-unmarked}
If $\co{X->right} = \co{null}$ then \co{X->status} is unmarked.
\end{lemma}
\begin{proof}
\Eric{This requires that we never call remove on the rightmost node in the list.  Once the algorithm calling remove is stabilized, check that that is true.  If not, we'll have to update this lemma and
its use to show that append preserves the invariant.  But note that \co{remove(B)} reads \B's right
neighbour's fields, so that would break if remove is called on the rightmost node in the list.}
\end{proof}

\begin{lemma}
\label{append-non-active}
When \co{tryAppend(A,B)} is called, \A\ is active and \B\ is not.
\end{lemma}
\begin{proof}
\Eric{This precondition of tryAppend should be trivial to check.  Maybe add that no other thread has a pointer to \B\ to ensure that \B\ is still inactive when the append CAS activates it.}
\end{proof}

\begin{figure}
\includegraphics[width=5in]{possibilities.jpg}
\caption{Possible configurations for consecutive non-finalized nodes \X\ and \Z.}
\label{possibilities}
\end{figure}

\begin{invariant}
\label{inv:list-invariant}
In any configuration, the following statements hold.
\begin{enumerate}
\item
\label{well-formed}
Consider the sequence of active, non-finalized nodes ordered by $<_c$.  If \X\ and \Z\ are two consecutive nodes in this sequence, then one of the following statements is true (refer to Figure \ref{possibilities}).
\begin{enumerate}[(a)]
\item 
\label{done}
$\X\leftrightarrow \Z$.
\item 
\label{not-done}
There is a finalized node \Y\ such that $\X\leftrightarrow \Y\leftrightarrow \Z$ and\\
a process has invoked \co{splice(X,Y,Z)}.
\item 
\label{left-done}
There is a finalized node \Y\ such that $\X\leftrightarrow \Y \rightarrow \Z$ and $\X \leftarrow \Z$ and\\
a process has invoked \co{splice(X,Y,Z)} and \\
no \co{splice(X,Z,*)} operation has completed line \ref{help-right-test}--\ref{help-right-cas}.
\item 
\label{right-done}
There is a finalized node \Y\ such that $\X\leftarrow \Y \leftrightarrow \Z$ and $\X \rightarrow \Z$ and\\
a process has invoked \co{splice(X,Y,Z)} and\\
no \co{splice(*,X,Z)} operation has completed line \ref{help-left-test}--\ref{help-left-cas}.
\end{enumerate}
\item
\label{splice-args}
If a \co{splice(U,V,W)} has been invoked before this configuration, then $\U\leftarrow \V \rightarrow \W$.
\item
\label{no-skip}
\begin{enumerate}[(a)]
\item
\label{no-skip-right}
If \X\ is finalized and $\X\rightarrow \Z$ then all nodes \Y\ such that $\X<_c \Y<_c \Z$ are finalized.
\item
\label{no-skip-left}
If \Z\ is finalized and $\X\leftarrow \Z$ then all nodes \Y\ such that $\X<_c \Y<_c \Z$ are finalized.
\Eric{This item will help show that a find won't skip any non-finalized nodes, and by Lemma \ref{remove-safe} that no non-removed nodes are skipped}
\end{enumerate}
\item
\label{unfinalized} 
If a \co{splice(U,V,W)} is in progress and \V\ is not finalized, then neither \U\ nor \W\ are finalized.
\Eric{I added this claim late.  Go through proof to see if it can be used to simplify any of the arguments}
\end{enumerate}
\end{invariant}

\Eric{Remark:  The property in the old proof that no reachable finalized node points to another finalized node is a trivial corollary of claim \ref{well-formed} of the invariant.  Proof:  Suppose not.  
I.e., there is a reachable finalized node that points to another finalized node.  Consider a path that reaches the first of these two.  Let \X\ be the last unfinalized node on this path.  \X\ exists since the head is never finalized.  Then \X\ points to a finalized node \Y\ that points to another finalized node.  This contradicts claim \ref{well-formed}.}

\Eric{Remark:  claim \ref{splice-args} implies that if \co{splice(A,B,C)} and \co{splice(A$'$,B,C$'$)} are called, then $\A=\A'$ and $\C=\C'$.}

\Eric{When proof is finished double-check that all claims of induction hypothesis are actually needed to make the proof go through.}

\begin{proof}
We first show that claim \ref{unfinalized} follows from the others.
To derive a contradiction, suppose claims \ref{well-formed}, \ref{splice-args} hold for some configuration but claim \ref{unfinalized} does not.
Then there is a \co{splice(U,V,W)} in progress such that \V\ is not finalized and either \U\ or \W\ is finalized.  
Without loss of generality, suppose \U\ is finalized (the other case is symmetric).
By claim \ref{splice-args}, $\U\leftarrow \V\rightarrow \W$.
Let \co{S} be the non-finalized node that precedes \V\ in the $<_c$ order.
Since the left pointer of the non-finalized node \V\ points to a finalized node \U, we are in case \ref{not-done} or \ref{right-done} of claim \ref{well-formed} for the consecutive
pair of non-finalized nodes \co{S}, \V.  Either way, a \co{splice(S,U,V)} has been invoked.
However, a \co{splice(U,V,W)} has also been invoked, contradicting Lemma \ref{no-overlap}.

It remains to show that for any step $s$ if all the claims are satisfied in all configurations before $s$, then claims \ref{well-formed}, \ref{splice-args} and \ref{no-skip} are satisfied in the configuration after $s$.
The only steps that can affect the truth of claims \ref{well-formed}--\ref{no-skip} are 
successful CAS steps, 
an invocation of \co{splice}, 
and completions of line \ref{help-left-test}--\ref{help-left-cas} or \ref{help-right-test}--\ref{help-right-cas} that do not perform a successful CAS. 
So, we will consider each of these types of steps in turn, after proving the following claim.

{\bf Claim:}  If, prior to $s$, two nodes \Y\ and $\Y'$ are finalized and there exist \X\ and \Z\ such
that \co{splice(X,Y,Z)} and \co{splice(X,Y$'$,Z)} have both been called, then $\Y=\Y'$.\\
{\bf Proof of claim:}
Any call to \co{splice(*,Y,*)} before $s$ must be \co{splice(X,Y,Z)}, by induction hypothesis \ref{splice-args}.  Thus, \Y\ was finalized by a call to \co{splice(X,Y,Z)}.
Similarly, $\Y'$ was finalized by a call to \co{splice(X,Y$'$,Z)}.
To derive a contradiction, suppose $\Y\neq\Y'$.
Without loss of generality, assume
\Y\ is finalized first.  Also, suppose $\Y<_c\Y'$ (the other case is symmetric).
In the configuration before \Y\ is finalized,
$\X\leftarrow \Y\rightarrow \Z$ by induction hypothesis \ref{splice-args}.
By induction hypothesis \ref{unfinalized}, \Z\ is not finalized.  
By induction hypothesis \ref{no-skip}, $\Z \leq_c \Y'$ since $\Y \rightarrow \Z$.
But we also have $\Y' <_c \Z$ since the call to \co{splice(X,Y$'$,Z)} implies $\Y'\rightarrow \Z$.
This contradiction completes the proof of the claim.

Now we show that each step preserves the invariant.

\begin{enumerate}[{C{a}se 1}]
\item
\label{right-cas-proof}
Suppose $s$ is a successful CAS at line \ref{right-cas} by a call to \co{splice(A,B,C)}.
This step changes $\co{A->right}$ from \B\ to \C.

To derive a contradiction, suppose \A\ is finalized in the configuration before $s$.
Consider the \co{splice(*,A,*)} operation that finalized \A.
By induction hypothesis \ref{splice-args}, since $\A\rightarrow\B$, it must have been a \co{splice(*,A,B)} operation.  This contradicts Lemma \ref{no-overlap}.
Thus, \A\ is not finalized when $s$ occurs.

By the test at line \ref{finalize-cas}, \B\ is finalized when $s$ occurs.
In the configuration before the CAS, we have $\A\leftarrow \B \rightarrow \C$ by induction hypothesis \ref{splice-args} and $\A \rightarrow \B$ since the CAS succeeds.
By induction hypothesis \ref{well-formed}, \C\ is not finalized and either $\A\leftarrow \C$ (case \ref{left-done}) or $\B\leftarrow C$ (case \ref{not-done}).
Thus, once $s$ updates \co{A->right} to \C, either case \ref{done} or \ref{right-done}, respectively, of claim \ref{well-formed} will be satisfied.

Next, we verify that $s$ preserves claim \ref{splice-args}.  Suppose \co{splice(U,V,W)} has been called before $s$.  The only way that $s$ can cause claim \ref{splice-args} to become false is if
it changes \co{V->right} from \W\ to another value.  If $s$ did this, it would have to be part of a 
\co{splice(V,W,*)} operation, but this would contradict Lemma \ref{no-overlap}.

Finally, we verify that $s$ preserves claim \ref{no-skip}.
This CAS updates \co{A->right} from \B\ to \C.  Since claim \ref{no-skip}\ref{no-skip-right} holds before $s$,
it suffices to check that there are no finalized nodes between \B\ and \C\ in the $<c$ order.
Prior to $s$, \B\ was finalized at line \ref{finalize-cas}, and $\B \rightarrow \C$, so by induction hypothesis \ref{no-skip}\ref{no-skip-right} there are no finalized nodes between \B\ and \C.

\item
\label{left-cas-proof}
Suppose $s$ is a successful CAS at line \ref{left-cas}.  This case is symmetric to \ref{right-cas-proof}.

\item
\label{help-right-cas-proof}
Suppose $s$ is a successful CAS at line \ref{help-right-cas} by a call to \co{splice(A,B,C)}.
This step changes $\co{A->right}$ from \D\ to \B, 
where \D\ is the value read from \co{A->right} at line \ref{help-right-read}.

Prior to the CAS, we have $\A\leftarrow\B$ by induction hypothesis \ref{splice-args},
and $\A\rightarrow \D$, since the CAS succeeds.
When the test at line \ref{help-right-test} was performed, $\D\rightarrow \B$.
Thus, we have $\A <_c \D <_c \B$.

Next, we prove that \B\ is not finalized when $s$ occurs.  To derive a contradiction, suppose \B\ is finalized before $s$.
By induction hypothesis \ref{splice-args} the operation that finalizes \B\
must be another \co{splice(A,B,C)} operation $sp$.
Let \E\ be the value read by $sp$ from \co{A->right} at line \ref{help-right-read}.
Since \co{A->right} is \D\ when $s$ later occurs, it follows from Lemma \ref{order} that $\E \leq_c \D$.
In the configuration when $sp$ reads \co{E->right} at line \ref{help-right-test},
we have $\A\leftarrow \B$ (by induction hypothesis \ref{splice-args}) and $\A<_c \E \leq_c \D <_c \B$.
At this point, \B\ is not yet finalized.   Since $\A\leftarrow \B$ and $\A\rightarrow \E$.
So, by induction hypothesis \ref{well-formed}, $\A\leftrightarrow \E\rightarrow \B$, \E\ is finalized,
and there has been a call to \co{splice(A,E,B)}.
When $sp$ reads \co{E->right} at line \ref{help-right-test}, it reads the value \B, by induction hypothesis \ref{splice-args}.
So, $sp$ performs the CAS at line \ref{help-right-cas}.
If this CAS succeeds, it would set \co{A->right} to \B\ prior to $s$.  
But in the configuration before $s$, $\A\rightarrow \D$ and $\D <_c \B$, contradicting Lemma \ref{order}.
Thus, the CAS performed by $sp$ at line \ref{help-right-cas} must fail.
So, the value of \co{A->right} changes from \E\ to some other value $\E'$ between $sp$'s read at line \ref{help-right-read} and $sp$'s CAS at line \ref{help-right-cas}.
Just after the CAS that makes this change, we have
$\A\rightarrow \E'$ and $\A\leftarrow \B$ and \B\ is not yet finalized.
So, by induction hypothesis \ref{well-formed}, $\E'$ is finalized and there has been a call to
\co{splice(A,E',B)}.
By the claim proved above, $\E=\E'$, which contradicts the definition of $\E'$.
Thus, \B\ is not finalized when $s$ occurs.

In the configuration before $s$, we have $\A\leftarrow \B$ and $\A\rightarrow \D$ and $\B$ is not finalized.
By induction hypothesis \ref{well-formed}, \A\ must not be finalized either, and \D\ must be finalized.

Consider the configuration $C_i$ when line \ref{help-right-read} is executed before $s$ and $\A\rightarrow \D$.  
By induction hypothesis \ref{splice-args}, $\A\leftarrow \B$ in $C_i$.
Since $\A<_c \D <_c \B$, \D\ must be finalized in $C_i$, by induction hypothesis \ref{well-formed}.
Let $C_j$ be the configuration before line \ref{help-right-test} is executed and $\D \rightarrow \B$.

To derive a contradiction, suppose \co{D->right} changes from \B\ to some other value \E\ between
$C_j$ and $s$.  Let $C_k$ be the configuration before this change occurs.
By Lemma \ref{order}, $\D<_c \B<_c \E$.
By induction hypothesis \ref{no-skip} applied to $C_{k+1}$,
\B\ must be finalized in $C_{k+1}$ (and hence also in $C_k$).
Since $\A\rightarrow \D$ holds in $C_i$ before $C_k$ and again after $C_k$ in the configuration before $s$,
it follows from Lemma \ref{order} that $\A\rightarrow\D$ in $C_k$.
So, in $C_k$ we have $\A\rightarrow \D\rightarrow \B$ and \A\ is not finalized, while \D\ and \A\ are finalized.  This contradicts induction hypothesis \ref{well-formed} for $C_k$.
Thus, our assumption is false and we have $\D\rightarrow \B$ in the configuration before $s$.

So, in the configuration before $s$, $\A\rightarrow \D\rightarrow \B$, $\A\leftarrow \B$, \A\ is not finalized,
and \D\ is finalized.
By induction hypothesis \ref{well-formed}\ref{left-done}, \B\ is not finalized and some process has called \co{splice(A,D,B)}.
Thus, in the configuration after $s$ we have $\A\leftrightarrow\B$, satisfying case \ref{done} of claim \ref{well-formed}.

To verify that $s$ preserves claim \ref{splice-args}, it must be shown that no \co{splice(*,A,D)} is in progress.
As argued above, \A\ is not finalized when $s$ occurs and there was a call to \co{splice(A,D,B)}.
Hence, by Lemma \ref{no-overlap}, there cannot be a call to \co{splice(*,A,D)}.

Finally, we verify that $s$ preserves claim \ref{no-skip}.
Let \D\ be the value of \co{A->right} in the configuration before $s$.
Then, $s$ updates \co{A->right} from \D\ to \B.
If \A\ is not finalized before $s$, then this step cannot make claim \ref{no-skip} false,
so suppose \A\ is finalized.
If \B\ is finalized, $\A\leftarrow \B$ by induction hypothesis \ref{splice-args}, so it follows from induction hypothesis \ref{no-skip} that there are no finalized nodes between \A\ and \B\ in the order $<_c$.
So, suppose \B\ is not finalized.
Then, in the configuration before $s$, \B\ is not finalized, but 
$\co{B->left->right} = \co{A->right} = \D \neq \B$ 
(the latter inequality follows from the fact that $\co{D->right} = \B$ 
at line \ref{help-right-test} so $\D<_c \B$ by Lemma \ref{order}).  
This contradicts induction hypothesis \ref{well-formed}
since, if a node \B\ is not finalized and \co{B->left} is finalized, then $\co{B->left->right} = \B$.

\item
\label{help-left-cas-proof}
Suppose $s$ is a successful CAS at line \ref{help-left-cas}.  This case is symmetric to \ref{help-right-cas-proof}.

\item
\label{finalize-cas-proof}
Suppose $s$ is a successful CAS at line \ref{finalize-cas} of \co{splice(A,B,C)} that finalizes \B.

To derive a contradiction, suppose \A\ is finalized before $s$.
$\A\leftarrow \B$ in the configuration before $s$ by induction hypothesis \ref{splice-args}.
Since \A\ is finalized but \B\ is not, induction hypothesis \ref{well-formed} implies that a \co{splice(*,A,B)} has been invoked.  This contradicts Lemma \ref{no-overlap}.
Thus, \A\ is not finalized in the configuration before $s$.

In the configuration before $s$, the two non-finalized nodes \A\ and \B\ with $\A\leftarrow \B$ cannot satisfy case \ref{left-done} of induction hypothesis \ref{well-formed}, since the \co{splice(A,B,C)} that performs $s$ has
completed lines \ref{help-right-test}--\ref{help-right-cas} before performing $s$.
So, they must satisfy case \ref{done}.

A symmetric proof shows that \B\ and \C\ are consecutive, non-finalized nodes that satisfy case \ref{done} of induction hypothesis \ref{well-formed} in the configuration before $s$.

Thus, when $s$ finalizes \B, \A\ and \C\ become consecutive, non-finalized nodes that satisfy case \ref{not-done} of claim \ref{well-formed}.

Step $s$ trivially preserves claim \ref{splice-args} since it does not change any \co{left} or \co{right} pointers.

Finally, we verify that $s$ preserves claim \ref{no-skip}.
In the configuration before $s$, \B\ is not finalized.
If \co{B->right} points to the next unfinalized node in the order $<_c$, then claim \ref{no-skip} is satisfied.
By induction hypothesis \ref{well-formed}, the only other possibility is that \co{B->right} is a finalized node whose \co{right} pointer is the next unfinalized node after \B\ in the order $<_c$.
In this case, again claim \ref{no-skip} is satisfied.

\item
\label{append-proof}
Suppose $s$ is a successful CAS at line \ref{append-cas} in \co{tryAppend}.
When this CAS modifies \co{A->right} from null to \B,
Lemmas \label{rightmost-unmarked} and \ref{append-non-active} imply that 
\A\ is active and unfinalized, and this CAS makes \B\ active, 
so \A\ and \B\ satisfy case \ref{not-done} of claim \ref{well-formed}.
This step does not affect the other claims of the invariant.


\item
\label{invoke-splice-proof}
Suppose $s$ is an invocation of \co{splice(U,V,W)}.  
This step does not affect the truth of claim \ref{well-formed} or \ref{no-skip}.  We must just verify that $\U\leftarrow \V\rightarrow \W$ to ensure claim \ref{splice-args} is satisfied.

We show that $\V\rightarrow\W$ in the configuration after $s$; the proof that $\U\leftarrow \V$ is symmetric.
By Lemma \ref{splice-precond}, there is an earlier time when $\V\rightarrow \W$.
To derive a contradiction, suppose there is some step $s'$ that changed \co{V->right} changed from \W\ to some other value \Z\ before $s$.
By Lemma \ref{order}, $\V <_c \W <_c \Z$.
Step $s'$ must be an execution of either line \ref{right-cas} or \ref{help-right-cas}.

Step $s'$ cannot be line \ref{right-cas}, since it would have to be inside a call to \co{splice(V,W,*)}, which contradicts Lemma \ref{no-overlap}.

So the change must be made at line \ref{help-right-cas} inside a \co{splice(V,Z,*)} operation.
To derive a contradiction, assume \V\ is finalized when $s'$ occurs.
The step that finalized \V\ was in a \co{splice(*,V,*)} operation.
Since $\V\rightarrow \Z$ in the configuration before $s'$, it must have been a \co{splice(*,V,Z)} operation, by induction hypothesis \ref{splice-args}.
This contradicts Lemma \ref{no-overlap}, since $s'$ is performed by a \co{splice(V,Z,*)} operation.
Thus, \V\ is not finalized when $s'$ occurs.

In the configuration after $s'$, we have $\V\rightarrow \Z$.  Since $\V <_c \W <_c \Z$, it follows from induction hypothesis \ref{well-formed} that \W\ is finalized when $s'$ occurs.
In the configuration before $s'$, we have $\V\rightarrow \W$, where \V\ is not finalized and \W\ is finalized.  By induction hypothesis \ref{well-formed}, $\V\leftarrow \W$.  Thus, by induction hypothesis
\ref{splice-args}, the \co{splice} operation that finalized \W\ must have been of the form \co{splice(V,W,*)}.  This contradicts Lemma \ref{no-overlap}, since $s$ is performed by a \co{splice(U,V,W)}.

Thus, no step $s'$ can change \co{V->right} from \W\ to any other value before $s$.  This completes the proof.

\item
\label{fail-help-right-proof}
Suppose $s$ is the completion of the if statement at line \ref{help-right-test}--\ref{help-right-cas} 
inside a \co{splice(X,Z,*)} operation without performing a successful CAS.
This means that either the test at line \ref{help-right-test} returns false or the CAS at line \ref{help-right-cas} fails.
We must show that \X\ and \Z\ are not in case \ref{left-done} of claim \ref{well-formed}.
To derive a contradiction, suppose that they are, i.e., in the configuration before $s$,
\X\ and \Z\ are not finalized,
there is a finalized node \Y\ such that $\X\leftrightarrow \Y\rightarrow \Z$,  $\X\leftarrow \Z$,
and a process has invoked \co{splice(X,Y,Z)}.
Let $s'$ be the execution of line \ref{help-right-read} prior to $s$ and let $\Y'$ be the value read from \co{X->right} at that line.
\Y\ cannot be $\Y'$, since then the test at line \ref{help-right-test} would return true (since 
$\Y\rightarrow \Z$ when $s$ occurs) and the CAS would succeed (since $\X\rightarrow \Y$ when $s$ occurs).

So, \co{X->right} must change from $\Y'$ to \Y\ between step $s'$ and $s$.
By Lemma \ref{order}, $\X <_c \Y' <_c \Y <_c \Z$.
By induction hypothesis \ref{splice-args}, $\X\leftarrow \Z$ when $s'$ occurs, since $s'$ is 
in a call to \co{splice(X,Z,*)}.
\X\ and \Z\ are not finalized at $s'$, since they are not finalized at the later step $s$.
By induction hypothesis \ref{no-skip}, $\Y'$ is finalized when $s'$ occurs.
By induction hypothesis \ref{well-formed}, when $s'$ occurs we have
$\X\leftrightarrow \Y' \rightarrow \Z$, and \co{splice(X,Y$'$,Z)} has been called.

Thus, in the configuration before $s'$, there have been invocations of \co{splice(X,Y$'$,Z)}
and \co{splice(X,Y,Z)}.  Moreover, \Y\ and $\Y'$ have both been finalized.
By the claim proved above, $\Y=\Y'$, 
which contradicts the fact that $\Y\neq \Y'$.  
This completes the proof for case \ref{fail-help-right-proof}.

\item
\label{fail-help-left-proof}
Suppose $s$ is the completion of the if statement at line \ref{help-left-test}--\ref{help-left-cas} without performing a successful CAS.  This case is symmetric to \ref{fail-help-right-proof}.


\end{enumerate}
\end{proof}

==> proof-progress.tex <==
\section{Proof of Progress}
\label{sec:proof_progress}

We say that a node is {\em reachable} in a list,
if it can be reached by following an arbitrary sequence of
$left$ or $right$ pointers of list nodes, 
starting from a list head node. We say that a node
is on the left of a node $X$ at $Q$ if we can reach it
by following  an arbitrary sequence of
$left$ or $right$ pointers of list nodes
starting with $X \rightarrow left$. 
Similarly, we say that a node is on the right of $X$ 
if we can reach it 
by following  an arbitrary sequence of
$left$ or $right$ pointers of list nodes
starting with $X \rightarrow right$. 

Consider any execution $\alpha$. For each configuration $Q$ in $\alpha$,
we define the {\em priority tree} at $Q$ to be a tree that contains all nodes
that are reachable at $Q$ and is constructed, {\em recursively}, as follows:
\begin{enumerate}
\item The root of the tree is the node $X$ with the highest priority among 
all reachable nodes at $Q$;
\item The left subtree is comprised by those nodes that are on the left of $X$;
\item The right subtree is comprised by those nodes that are on the right of $X$;
\end{enumerate}
\here{Youla: the definition above assumes that  the priorities are distinct. 
If they are not, as is the case in our algorithm, we need to also explain
how t obreak ties. This should be done carefully, so that the lemmas below
still hold.}

For each configuration $Q$, we denote by $T_Q$ the priority tree at $Q$.
By the way the priority tree is constructed, the following holds:

\begin{observation}
\label{obs:priorities}
Consider any configuration $Q$ and let $X$ be any node in $T_Q$.
Then, $X$ has higher priority than all of its descendants in $T_Q$.
\end{observation}

\begin{lemma}
\label{lem:prtree}
Consider two subsequent configurations $Q$ and $Q'$ in $\alpha$
and let $X, Y$ be two nodes that belong to both $T_Q$ and $T_{Q'}$,
such that $Y$ is a descendant of $X$ in $T_Q$. 
Then, $Y$ is a descendant of $X$ in $T_{Q'}$.
\end{lemma}

\begin{proof}
There are three CAS instructions in the pseudocode that may cause the priority tree
to change. The first is the CAS of line~\ref{append-cas} (that appends a node in the list),
the second is the CAS of line~\ref{right-cas}, and the third is the CAS of line~\ref{left-cas}
in case $A = NULL$. We consider each of these CAS steps separately. 

\begin{enumerate}
\item Assume first that the instruction executed from $Q$ to get $Q'$ is a CAS instruction of line~\ref{append-cas} that appends a node $B$ in the list. 
By inspection of the pseudocode, the CAS of line~\ref{append-cas} is successful only if its old parameter
is equal to NULL. By inspecting the pseudocode, it follows that all new nodes 
inserted in the list, are appended at the right endpoint of the list. 
Therefore, the subtree that will emanate from $B$ in $T_{Q'}$ will have a single left
subtree (as $B$ does not have any nodes on its right at $Q'$). 
Moreover, $B$ will be the right child of a node $A$ in $T_Q$ and the right subtree of $A$ in $T_Q$ 
will be the left subtree of $B$ in $T_{Q'}$. (Note that $A$ will be the first reachable node in the list with the smallest
priority that is higher than the priority of $B$ among those we traverse when
we start from the right endpoint of the list and move leftwards.) These changes do not violate the claim.

\item  Assume now that the instruction executed from $Q$ to get $Q'$ 
is a CAS instruction either of line~\ref{right-cas}, or of line~\ref{left-cas} (with $A = NUUL$),
that makes a node $B$ unreachable.
Let $A$ be the parent of $B$ in $T_Q$ and let $D$ and $E$ be its children. 
Wlog, assume that $B$ is a left child of $A$ and that the priority of $D$ is larger than that of $E$
(the other cases are symmetr,ic).

Observation~\ref{obs:priorities} implies that the node with the highest priority on the right
of $A$, after $B$ is removed, is $D$, the child of $B$ with the highest priority.
By the way the priority tree is constructed, it follows that the left child of $A$ in $T_{Q'}$ is $D$. 
The left subtree of $D$ is the same in both $T_Q$ and $T_{Q'}$. For the right subtree of $D$
the following hold: 1) $E$ is the root of this subtree; 2) the right subtree of $E$ will stay intact;
3) the left subtree of $E$ will be a merged version of the right subtree of $D$ and the left subtree
of $E$. By Observation~\ref{obs:priorities}, for every pair of nodes $X,Y$ such that $Y$ is an ancestor
of $X$ in $T_Q$, the priority of $Y$ is higher than the priority of $X$. By the way the tree is constructed,
it follows that $Y$ will be placed as a descendant of $X$ in the merged subtree that will comprise
$E$'s left subtree. 

From all the above, it follows that the claim holds.

\here{Youla: What I write here is true if the priorities are unique. If they are not, we need
to define the priority tree more carefully and also be more careful in our argumentation.}
\Hao{The argument above works even if we splice out a node in the implicit tree with two children.}
\Hao{We need to prove a height bound on the implicit tree.}
%
%\item Similar to previous case (actually simpler).
\end{enumerate}
\end{proof}

%Corollary~\ref{} is an immediate consequnce of Lemma~\ref{lem:prtree}.

\begin{corollary}
\label{cor:prtree}
Consider two configurations $Q$ and $Q'$ in $\alpha$ with $Q$ preceeding $Q'$,
and let $X, Y$ be two nodes that belong to both $T_Q$ and $T_{Q'}$.
If $Y$ is a descendant of $X$ in $T_Q$, then $Y$ is a descendant of $X$ in $T_{Q'}$.
\end{corollary}


We say that a routine is {\em active} at $Q$, if it has been invoked but it has not yet returned.

\begin{lemma}
\label{lemma:implicit tree}
For each configuration $Q$, if a node $B$ with $B \rightarrow status \neq unmarked$
is reachable, then one of the following holds:
\begin{enumerate}
\item there exist an active instance of either remove(B) or remove\_rec(B), 
or remove(D) or remove\_rec(D), where $D$ is a descendant of $B$ in $T_Q$, or
\item if $A = B \rightarrow left$, $C = B \rightarrow right$,
and $a, b, c$ are the priorities of $A, B, C$, respectively,
then $a < b > c$.
\end{enumerate}
\end{lemma}

\begin{proof}
Consider any reachable node $B$ with $B \rightarrow status \neq unmarked$ at $Q$.
To derive a contradiction, assume that the claim does not hold.
Since $B \rightarrow status \neq unmarked$, $B \rightarrow status$ is either $marked$ or $finalized$. 
\begin{enumerate}
\item
Assume first that $B \rightarrow status$ is finalized at $Q$. As the $status$
of a node may change only if a successful CAS\ of line~\ref{finalize-cas} is executed, 
an instance $I_s$ of splice(*,B,*) has been called by $Q$. Invariant~\ref{inv:correctness}
implies that $I_s$ is still active at $Q$, as otherwise $B$ would not be reachable at $Q$. 
		By inspection of the pseudocode, $I_s$ is called either by an instance of remove\_rec($B$) or by an instance of help(). 
Denote by $I$ this instance. Note that $I$ is still active at $Q$ (since $I_s$ that 
it invokes is still active at $Q$). 
If $I$ is an instance of remove\_rec($B$), the claim holds. 
		
Assume that $I$ is an instance of help(). By inspection of the pseudocode, it follows that $I$ 
is called either on line~\ref{remove-help}, or on line~\ref{sul-help}, or on line~\ref{sur-help}.	
If $I$ is called on line~\ref{sul-help}, 
an instance of SpliceUnmarkedLeft(*, B, *) is active. This instance has been called 
by an instance of remove\_rec(B) which is still active. So, the claim holds. 
The case that $I$ is called on line~\ref{sur-help} is symmetric.

Assume now that $I$ is called on line~\ref{remove-help} by an instance $I_r$ of remove($X$)
for some node $X$. Since $I$ calls splice(), it must be that 
the condition of line~\ref{test-frozen} is evaluated to TRUE.
By inspection of the pseudocode, it follows that a descriptor, $desc$, 
containing $\{*, B, * \}$ has been installed into a node $Y$.
Wlog, assume that $desc$ is stored in $X \rightarrow rightDesc$ (the case
where $desc$ is stored in $X \rightarrow leftDesc$ is symmetric).
As descriptors are installed into a node's $rightDesc$ field only on line~\ref{store-right-desc} %and~\ref{store-left-desc},
it follows that there is an instance $I_{su}$ of spliceUnmarkedLeft($X, B, *$)
%or spliceUnmarkedRight($*, B, X$) 
that has installed $desc$. By inspection of the pseudocode,
it follows that this instance has been invoked by an instance $I_{rr}$ of remove\_rec($B$).
It suffices to argue that $I_{rr}$ is still active at $Q$. To derive a contradiction,
assume that this is not so. 

Recall that by assumption only one instance of remove() is called on each node,
thus $I_r$ is the only instance of remove($X$) that is invoked in $\alpha$.
By inspection of the pseudocode,
it thus follows that $desc$ can become frozen only by $I_r$.
Since $I$ calls $I_s$, it therefore follows that $desc \neq frozen$ as long as $I$ is active,
and threfore $desc \neq frozen$ at $Q$.  

Note that $I_{su}$ also calls help($desc$) (line~\ref{sul-help}),
right after installing $desc$ into $X \rightarrow leftDesc$ (line~\ref{store-left-desc}). 
Let $Q'$ be the configuration at which the instance of help($desc$)
called by $I_{su}$ evaluates the condition of line~\ref{test-frozen}. 
Recall that when a $desc$ becomes frozen it remains frozen forever. 
		Since $I_{rr}$ is not active at $Q$ (by assumption),
and $desc \neq frozen$ at $Q$, it follows that $I_{su}$ evalautes the
condition of line~\ref{test-frozen} to TRUE,
		and thus it invokes splice($*,B,*$). Since $I_{rr}$ is not active
at $Q$, this instance of splice has been completed by $Q$. 
By Invariant~\ref{inv:correctness}, it follows that $B$ is not reachable at $Q$. 
This is a contradiction. 

\here{Youla: Have we proved in the correctness part that "If an instance of splice(A,B,C) 
completes, then $B$ is not reachable any longer"? I mean that this is so independently
of whether splice returned TRUE or FALSE. I need such a lemma here, if we do not have it.}
%I also need the following: "When help(desc) is first called with $desc \neq null$,
%then it invokes splice()".








\item Assume now that $B \rightarrow status$ is $marked$ at $Q$. Then, some instance $I_r$ of remove($B$) has been called
at some configuration prior to $Q$. If $I_r$ is active at $Q$, the claim holds. 

Assume that $I_r$ is not active at $Q$. By inspection of the pseudocode, 
it follows that $I_r$ invokes an instance $I_{rr}$ of remove-rec($B$).
If $I_r$ called splice() on line~\ref{}, this splice() is completed. Invariant~\ref{inv:correctness} implies that 
$Y$ is no longer reachable. A contradiction.
So, assume that splice() was not called. Then, either an instance $I_s$ of either spliceUnmarkedLeft(*,Y,*) or
of SpliceUnmarkedRight(*,Y,*) was invoked. Assume, wlog, that  $I_s$ is an instance of 
spliceUnmarkedLeft(*,Y,*) (the other case is symmetric). 

What if no such instance is invoked? I still have to argue about this case. 
\end{enumerate}
\end{proof}


==> proof-youla.tex <==
% !TEX root =  main.tex

\newpage

\section{Algorithm of Figure~\ref{break-ties}: Proof of Correctness}


\Eric{This section contains two alternate formalizations of the same result}

We say that a node is {\em reachable},
if it can be reached by following an arbitrary sequence of
$left$ or $right$ pointers of nodes, 
starting from the head node.
Note that a node has two pointers, $left$ and $right$. 
Let $ptr$ be a pointer of a node $X$ (i.e., $ptr$ is either the $left$ or the $right$ pointer of $X$)
and let $Y$ be the node to which $ptr$ points. 
We say that $ptr$ is {\em valid}, if the following hold: 
if $ptr = X \rightarrow left$ then $Y \rightarrow right$ points to $X$, 
otherwise, $Y \rightarrow left$ points to $X$.
For every node $X$, we call the node that $X \rightarrow left$ points to $X$'s {\em left neighbor}
and the node that $X \rightarrow right$ points to $X$'s {\em right neighbor}.

We assume that initially, all nodes in the chain are not {\em finalized}, 
i.e., their \emph{state} field is not equal to finalize. We also assume
that they are distinct and  all their pointers are valid. 
We also assume that all nodes are distinct.

Consider any execution $\alpha = C_0, s_1, C_1, s_2, C_2, \ldots$. 
For each $i \geq 0$, denote by $V_i$ the set of nodes that are in finalized state
at configuration $C_i$ and can be accessed by one of the endpoints of the chain. 
Note that $V_0 = \emptyset$, as no node is finalized at $C_0$.

The following is an immediate consequence of the code and the fact that 
the node priorities are immutable.

\begin{observation}
Consider any instance $I_s$ of splice() with parameters, $W,X,Y$. 
If $w,x,y$ are the priorities of $W,X,Y$, it holds that $w > x < y$.
\end{observation}


%\begin{observation}
%Consider any  instance $I_s$ of splice() with parameters, $W,X,Y$. 
%Let $I_r$ be the instance or remove\_rec() that calls $I_s$. 
%Then, $W = X->left$ and $Y = X->right$ from the time that 
%each is read on line 21 or 22 and the time that $X$ is finalized.
%\end{observation}


\begin{theorem}
For every $i \geq 0$, the following hold at configuration $C_i$.
	\begin{enumerate}
		\item If $X$ is a reachable finalized node, then: 
\begin{enumerate}
\item The node  $W = X \rightarrow left$ and the node $Y = X \rightarrow right$ are not in state finalized;
	\label{finalize}
\item If w,x,y, are the priorities of $W,X,Y$, respectively, then $w > x < y$;
	\label{order}
\item $W$ and $Y$ were the nodes pointed to by the $left$ and $right$ pointers of $X$ since $X$ was finalized;
	\label{X neighbors}
\item either ($W \rightarrow right  = X$ and $Y \rightarrow left = X$) or ($w>y$ and $W \rightarrow right = Y$ and $Y \rightarrow left = X$) 
	or ($y>w$ and $Y \rightarrow left = W$ and $W \rightarrow right = X$);
	\label{W and Y neighbors} 
\end{enumerate}
\item  let $P$ be the set of pointers of all reachable nodes, and let $P'$ be a set of pointers such that 
	for every reachabe node $Z$ that is finalized, $P'$ contains the two pointers of $Z$, the left pointer of $Z$'s right neighbor 
		and the right pointer of $Z$'s left neighbor. Then, every pointer in $P \setminus P'$ is valid; \label{rest}
\item all nodes that have been inserted in the chain and are not in finalized state are reachable; \label{reachable}
\item all nodes that have been inserted in the chain and have been unreachable in some configuration before $C_i$
	are still unreachable. \label{unreachable}
%\item the chain contains no cycles.\label{no cycles}
%\item all nodes are distinct. \label{distinct}
\end{enumerate}
\end{theorem}

\begin{proof}
By induction on $i$. Note that the only instructions that may change the invariant
are the CAS instructions on lines 36,39,40,43,44, and insertions in the list. 
Insertions occur only at  the one end of the list. Moreover, the new nodes 
	are distinct, not finalized, and (once inserted in the list) their pointers are valid. So, insertions maintain the invariant. 

\noindent
{\bf Base Case ($ i = 0$).}
For $i = 0$ the claim holds vacaously, as $V_0 = \emptyset$
and all nodes in the chain are distinct, non-finalized, and their pointers are valid. 

\noindent
{\bf Induction Hypothesis.} Consider any $i >0$ and assume that 
the invariant holds at $C_{i-1}$.

\noindent
{\bf Induction Step.} We prove that the invariant holds at $C_i$.
If $s_i$ is not a successful CAS step, then the invariant holds
by induction hypothesis. 
So, assume that $s_i$ is a successful CAS step.
Let $W',X,Y'$ be the parameters of the instance, $I_s$, of splice()
that executes $s_i$, and let $I_r$ be the instance of remove\_rec() that executes $I_s$. 
%Assume that $X$ is a reachable node at $C_{i-1}$, as otherwise the invariant holds
%at $C_i$ be the induction hupothesis.
By inspection of the code, it follows that $X$ is finalized at $C_i$.
Note that if $X$ is not reachable at $C_{i-1}$, then the claims hold by induction hypothesis 
(this requires some argumentation but I think it is easy to see why it holds). 
So, assume that $X$ is reachable at $C_{i-1}$. 
%We can also easily prove that when a node becomes unreachable, it stays unreachable forever.
We prove that the invariant holds for $X$.
%It also follows that $w' > x < y'$ (because of the test of line 23),
%where $w'$ and $y'$ are the priorities assigned to $W'$ and $Y'$, respectively.
We first prove:

\begin{lemma}
\label{not finalized}
Neither $W'$ nor $Y'$ is finalized at $C_i$.
\end{lemma}

\begin{proof}
By inspection of the code, it follows that $W' = X \rightarrow left$ when line 20 
of $I_s$ is executed and $Y' = X \rightarrow right$ when line 21 is executed. 
Recall that the priorities of nodes are immutable. 
So, the test on line 23 implies that $w' > x < y'$, where $w'$ and $y'$ are the priorities
of $W'$ and $Y'$, respectively. 

%We argue that neither $Y$ nor $W$ is finalized at $C_i$. 
%To prove Claim~\ref{finalize}, 
To derive a contradiction, assume that one of the $Y'$, $W'$ is finalized at $C_i$.
Wlog, assume that it is $Y'$ that is finalized. 
%Note that when a reachable node becomes unreachable, it never becomes reachable again.
%Since $X \in V_i$, $X$ is reachable at $C_i$ and therefore, 
Recall that $X$ is reachable at $C_{i-1}$ and that as soon as a node becomes unreachable
it remains unreachable forever. Thus, $X$ was reachable when $Y'$ and $W'$
were read. Thus, $Y'$ and $W'$ were also reachable at those points in time.
The induction hypothesis (Claims~\ref{W and Y neighbors} and~\ref{rest}) implies that the chain contains no cycles at $C_{i-1}$.
As all nodes are distinct, these imply that $X \neq Y'$ and $X \neq W'$. 
Note that if $s_i$ is a CAS of line 36, it finalizes the state of $X$.
It follows that there exists
a configuration $C_j$ before $C_i$ ($j<i$) at which the state of $Y'$ is finalized. 
By inspection of the code, it follows that when the state of a node becomes
finalized, it remains finalized "forever". Thus, the state of $Y'$ is finalized
between $C_j$ and $C_i$. 

At $C_j$, $Y' \in V_j$, so by induction hypothesis, if $X'$ and $Z$ are the neighbors
of $Y'$ at $C_j$ then none of them is finalized at $C_j$ and $x' > y' < z$ at $C_j$. 
Since $x < y'$, these imply that $X \neq X'$ and $X \neq Z$. 
So, $X$ is not the left neighbor of $Y'$ at $C_j$. There are two ways that 
$X$ can become a neighbor of $Y'$. 1) It is a newly inserted node in the list.
	Then, it should be easy to reach a contradiction.
2) $Y'  \rightarrow  left$ changes to point to $X$ between $C_j$ and $C_i$. 
This can only occur by executing the CAS of either line 40 or 43.
When this CAS is performed, $Y' \rightarrow left$ points to a finalized node
and $Y'$ is also finalized. This is a contradiction to induction hypothesis (Claim~\ref{finalize}).
It follows that neither $Y'$ nor $W'$ are finalized at $C_i$. 
\end{proof}

\begin{lemma}
\label{no change}
$X \rightarrow left$ points to $W'$ and $X \rightarrow right$ points to $Y'$ at $C_i$, i.e., $W' = W$ and $Y' = Y$.
\end{lemma}

\begin{proof}
To derive a contradiction, assume that the claim does not hold.
Wlog, assume that $X \rightarrow right$ does not point to $Y'$ at $C_i$. 
Let $C$ be the configuration at which $X \rightarrow right$ is read and
is assigned to $Y'$ in $I_s$. 
By inspection of the code, there should be a configuration 
between $C$ and $C_i$, where a CAS of either line 39 or 44 is executed
to change $X \rightarrow right$. Consider the first such CAS. 
By the time this CAS is executed, $X \rightarrow right$ points
to $Y'$. Since the CAS is successful, it changes $X \rightarrow right$ from $Y'$
to point to some other node. By inspection of the code, it should
be that $Y'$ is finalized when the CAS is executed. Since the CAS is executed
before $C_i$ and when a node is finalized remains finalized forever, 
$Y'$ is finalized at $C_i$. This contradicts Lemma~\ref{not finalized}.
\end{proof}

We proceed by case analysis.
\begin{enumerate}
\item $s_i$ is a successful CAS step of line 36. 
Then, $V_i = V_{i-1} \cup \{X\}$. 
		Lemma~\ref{no change} implies that $W' = X \rightarrow left$ and $Y' = X \rightarrow right$ at $C_i$. 
		Lemma~\ref{not finalized} implies that neither $X \rightarrow right$ nor $X \rightarrow left$ is finalized at $C_i$,
		as needed for Claim~\ref{finalize}.
%Recall that $X \rightarrow right$ ($X \rightarrow left$) pointed to $Y$ ($W$, respectively) when
%line 21 (20, respectively) were executed. Since $X$ is not finalized when these
%lines are executed, the induction hypothesis (claim~ref{rest})
%		implies that $Y->left = X$ ($W->right =X$) when line 21 (20)
%		is executed. By inspection of the code, from this point onwards, 
%		the only way for $Y->left$ and $W->right$ to change
%		is if $X$ is finalized and the CAS of line 
%
%		$X -> right$ points to $Y$ and $X->left$ points to $W$, and $X$ is reachable
%at $C_{i-1}$, it follows that 
%By inspection of the code, it follows that 
The rest of the claims hold by the induction hypothesis. 


\item $s_i$ is a successful CAS step of line 39. 
Lemma~\ref{no change} and the code imply that $X \rightarrow left$ points to $W' = W$ at both $C_{i-1}$ and $C_i$, and that $Y' = Y$.
		By the test on line 38, $w>y$. Since the CAS is successful, $W \rightarrow right$ points to $X$ at $C_{i-1}$. 
		By induction hypothesis (Claim~\ref{W and Y neighbors}, it therefore holds that 
		$W \rightarrow right = X$ and $Y \rightarrow left = X$ at $C_{i-1}$. It follows that at $C_i$,
		it holds that ($w>y$ and $W \rightarrow right = Y$ and $Y \rightarrow left = X$), as needed by Claim~\ref{W and Y neighbors}.
		Note that no node becomes unreachable because of the execution of $s_i$. 

		The rest of the claims can be derived easily by the induction hypothesis. 
	
\item $s_i$ is a successful CAS step of line 43. This case
	is symmetric to the previous one. 

\item $s_i$ is a successful CAS step of line 40. 
Lemma~\ref{no change} and the code imply that $X \rightarrow right$ points to $Y' = Y$ at both $C_{i-1}$ and $C_i$;
moreover, $X \rightarrow left$ points to $W' = W$ at all  times between $X$'s finalization and $C_i$. 
By the test on line 38, $w > y$. Since the CAS is successful, $Y \rightarrow left$ points to $X$ at $C_{i-1}$. 
To prove Claim~\ref{W and Y neighbors}, it suffices to prove that $W \rightarrow right = Y$ at $C_{i-1}$ (and therefore also at $C_i$). 
We first argue that there is a configuration between the configuration that finalized $X$ and
$C_{i-1}$ at which $W \rightarrow right$ is set to point to $Y$. 
By inspection of the code, $I_s$ executes the CAS of line 47 before $s_i$ and after $X$ becomes finalized. 
Let $cs$ be the first CAS that is executed by any instance of splice() with 
parameters $W,X,Y$. It is easy to argue that it succeeds and thus it changes $X \rightarrow right$ to point to $Y$. 
We next argue that no further change of $W \rightarrow right$ occurs between $cs$ and $C_i$. 
To derive a contradiction, assume that this is not the case. 
Then, a CAS of line either 47 or 52 change $W \rightarrow right$ to point to another node. 
Assume the first of this CAS, which changes $W \rightarrow right$ to point from $Y$ to a node $Z$. 
		When this CAS is executed, it must be that $Y$ is finalized. This contradicts Claim~\ref{finalize}
		of the induction hypothesis. It follows that $W \rightarrow right$ points to $Y$ at $C_{i-1}$.

By induction hypothesis (Claim~\ref{W and Y neighbors}, it holds that 
$W \rightarrow right = Y$ and $Y \rightarrow left = X$ at $C_{i-1}$. It follows that at $C_i$,
$X$ is no longer reachable, $W \rightarrow left$ points to $Y$ and $Y \rightarrow right$ points to $X$. 
		This and the induction hypothesis imply that Claims~\ref{rest} and~\ref{reachable} hold at $C_i$. 
		Note that $V_i = V_{i-1} \setminus \{ X\}$. Thus, 
		the rest of the claims follow by the induction hypothesis. 

\item $s_i$ is a successful CAS step of line 44. This case
	is symmetric to the previous one. 
\end{enumerate}

Since $s_i$ may change either the state of $X$, or the $right$ pointer of $W$ or the $left$ pointer of $Y$,
and both $W$ and $Y$ are not finalized at $C_i$, it follows that for all other nodes in $V_i$,
the invariant holds by the induction hypothesis. 

\end{proof}
=======

\Eric{Here is where the second version of this section begins}

We say that a node is {\em reachable},
if it can be reached by following an arbitrary sequence of
$left$ or $right$ pointers of nodes, 
starting from the head node.

\Eric{I'm abusing notation to use $X$ both to talk about a node and a pointer to a node}

\Eric{I needed to use different letters for the proof than the ones used in the algorithm for the three nodes.  So I'd like to rename the three arguments of splice in the code to ABC}

\Eric{There are some bits of the proof that are slightly repetitive that might be possible to clean up by linking claims 2 and 5 more closely}

\begin{lemma}
For any configuration, 
\begin{enumerate}
\item
\label{non-adjacent}
If $X$ is a reachable, finalized node then neither $X\rightarrow right$ nor $X\rightarrow left$ is finalized.
\item
\label{priorities}
If $X$ is a reachable, finalized node then $X\rightarrow left\rightarrow priority > X\rightarrow priority < X\rightarrow right\rightarrow priority$.
\item
\label{right-consistent}
If $X$ is a reachable node and $X\rightarrow right = Y$ then either
\begin{itemize}
\item 
$Y\rightarrow left = X$,
\item 
$X$ is finalized and 
$Y\rightarrow left = X\rightarrow left$ and \\
$Y\rightarrow priority > Y \rightarrow left\rightarrow priority > X\rightarrow priority$, or
\item 
there is a finalized $Z$ such that $Y\rightarrow left = Z$ and 
$Z\rightarrow left = X$ and \\
$X\rightarrow priority > Y\rightarrow priority > Z\rightarrow priority$.
\end{itemize}
\item
\label{left-consistent}
If $X$ is a reachable node and $X\rightarrow left = W$ then either
\begin{itemize}
\item 
$W\rightarrow right = X$,
\item 
$X$ is finalized and 
$W\rightarrow right = X\rightarrow right$ and \\
$W\rightarrow priority > W \rightarrow right\rightarrow priority > X\rightarrow priority$, or
\item 
there is a finalized $Z$ such that $W\rightarrow right = Z$ and 
$Z\rightarrow right = X$ and \\
$X\rightarrow priority > W\rightarrow priority > Z\rightarrow priority$.
\end{itemize}
\item
\label{pending-splice}
If a splice($W,X,Y$) operation is in progress then $X\rightarrow left=W$ and $X\rightarrow right=Y$.
\item
\label{still-reachable}
If $X$ is a node that has been appended to the list and $X$ is not finalized, then $X$ is still reachable.
\end{enumerate}
\end{lemma}

\begin{proof}
The claim is true in the initial state.

Suppose the invariant holds in some configuration $C_i$.  We prove that it is true in the next configuration $C_{i+1}$.  Let $s$ be the step that goes from $C_i$ to $C_{i+1}$.
We need only consider steps $s$ that are successful CAS steps.

\bigskip

{\bf Case 1}:  $s$ is a successful CAS that finalizes some node $B$.

Step $s$ trivially preserves claims \ref{right-consistent}, \ref{left-consistent}, \ref{pending-splice} and \ref{still-reachable}.

We must check that claim \ref{priorities} is satisfied for $X=B$ in $C_{i+1}$.  Since $s$ is performed by a splice$(A,B,C)$, it follows from the test on line \ref{test-priority} that $A\leftarrow priority > B\leftarrow priority < C\leftarrow priority$. Induction hypothesis \ref{pending-splice} implies that $B\rightarrow left = A$ and $B\rightarrow right =C$, so claim \ref{priorities} follows.

There are two ways that $s$ could cause a violation of claim \ref{non-adjacent}:  $B\rightarrow right$ or $B\rightarrow left$ could already be finalized, or there could be a reachable, finalized node $X$ such that $X\rightarrow right$ or $X\rightarrow left$ is $B$.  We show that neither of these can occur.

First, suppose the node $C=B\rightarrow right$ is already finalized in $C_i$.  
(The case where $B\rightarrow left$ is finalized in $C_i$ is symmetric.)
By induction hypothesis \ref{non-adjacent}, $C\rightarrow left$ is not finalized in $C_i$.
By induction hypothesis \ref{right-consistent}, $C\rightarrow left$ is $B$ (since neither $B$ nor $C.left$ is finalized in $C_i$).
By induction hypothesis \ref{priorities}, $B\rightarrow priority = C\rightarrow left\rightarrow priority > C\rightarrow priority$.
By induction hypothesis \ref{pending-splice}, $s$ is performed by a call to splice$(*,B,C)$.
So by the test on line \ref{test-priority}, $B\rightarrow priority < C\rightarrow priority$, a contradiction.

Now, suppose there is a reachable node $X$ that is finalized in $C_i$ and has $X\rightarrow right = B$.
(The case where $X\rightarrow left=B$ is symmetric.)
By induction hypothesis \ref{priorities}, $X\rightarrow priority < B\rightarrow priority$.
By induction hypothesis \ref{right-consistent}, there are three possibilities.
\begin{itemize}
\item
$B\rightarrow left = X$.  By induction hypothesis \ref{pending-splice}, $s$ is performed by a call to splice($X,B,*$).  By the test on line \ref{test-priority}, $X\rightarrow priority > B\rightarrow priority$, a contradiction.
\item
$X$ is finalized and $B\rightarrow left = X\rightarrow left$ and $B\rightarrow priority > X\rightarrow priority$.  The latter inequality is again a contradiction.
\item
There is a finalized $Z$ such that $B\rightarrow left = Z$ and $Z\rightarrow left = X$.  Since $Z$ and $X$ 
are both finalized in $C_i$, this would contradict induction hypothesis \ref{non-adjacent}.
\end{itemize}

\bigskip
{\bf Case 2}:  $s$ is a successful CAS on line \ref{right-cas1} that changes $A\rightarrow right$ from $B$ to $C$.

To show that $s$ preserves claim \ref{non-adjacent}, it is sufficient to show that it is preserved for $X=A$, i.e., if $A$ is reachable in $C_{i+1}$, then $C$ is not finalized in $C_{i+1}$.
Suppose $A$ is reachable in $C_{i+1}$ (and therefore in $C_i$).
By induction hypothesis \ref{pending-splice}, $B\rightarrow right = C$ in $C_i$.
Prior to performing $s$ at line \ref{right-cas1}, $B$ was finalized at line \ref{finalize-cas}, so $B$ is finalized in $C_i$.
Since $A$ is reachable in $C_i$ and $A\rightarrow right=B$, $B$ is also reachable in $C_i$.
By induction hypothesis \ref{non-adjacent}, $C=B\rightarrow right$ is not finalized in $C_i$.

To show that $s$ preserves claim \ref{priorities}, it is sufficient to show that $A$ is not reachable and finalized in $C_{i+1}$.
Suppose $A$ is reachable in $C_{i+1}$ (and therefore in $C_i$).
By induction hypothesis \ref{pending-splice}, $B\rightarrow left =A$ in $C_i$.
Prior to performing $s$ at line \ref{right-cas1}, $B$ was finalized at line \ref{finalize-cas}, so $B$ is finalized in $C_i$.
Since $A$ is reachable in $C_i$ and $A\rightarrow right=B$, $B$ is also reachable in $C_i$.
By induction hypothesis \ref{non-adjacent}, $A=B\rightarrow left$ is not finalized in $C_i$.

To show that $s$ preserves claim \ref{right-consistent}, we need only consider the node $X=A$.
We show that in $C_{i+1}$, the third bullet of claim 3 is satisfied with $Z=B$.
$B$ is finalized in $C_{i+1}$, since the CAS at line \ref{finalize-cas} prior to $s$ succeeded.
Since the test on line \ref{priority-switch} was true, we have $A\rightarrow priority > C\rightarrow priority$.  
Since $s$ is performed by a call to splice($A,B,C$), $C\rightarrow priority > B\rightarrow priority$, by the test on line \ref{test-priority}.
By induction hypothesis \ref{pending-splice}, $B\rightarrow right = C$ in $C_i$.
Since $A\rightarrow priority > C\rightarrow priority > B\rightarrow priority$, it follows from induction hypothesis \ref{right-consistent} that $C\rightarrow left = B$.
By induction hypothesis \ref{pending-splice}, $B\rightarrow left = A$.
This completes the proof of claim \ref{right-consistent}.

To show that $s$ preserves claim \ref{left-consistent}, we show that each of the bullets is preserved.

The first bullet can only become false if $W=A$ and $X=B$, i.e., if $B\rightarrow left =A$.
In this case, we show that the second bullet becomes true in $C_{i+1}$.
$B$ is finalized by line \ref{finalize-cas} before $s$ is executed at line \ref{right-cas1}.
By induction hypothesis \ref{pending-splice}, $B\rightarrow right =C=A\rightarrow right = C$
in $C_{i+1}$.
By the test in line \ref{priority-switch}, $A\rightarrow priority > C\rightarrow priority$ and by induction hypothesis \ref{priorities}, $C\rightarrow priority > B\rightarrow priority$.

The second bullet could become violated as a result of $s$ if either $W=A$ or $X=A$.
Since $s$ is performed by a splice($A,B,C$) operation, induction hypothesis \ref{pending-splice} implies that $B\rightarrow left =A$.  Since $B$ is finalized in $C_i$, induction hypothesis \ref{non-adjacent} implies that $A$ is not finalized in $C_i$.  This means that the second bullet could not have been true in $C_i$ with $X=A$.  So, it remains to consider the case where $W=A$.
To derive a contradiction, suppose the second bullet is satisfied for some reachable node $X$ and $W=A$ in $C_i$.
Then in $C_i$, $X\rightarrow right = A\rightarrow right = B$ and both $X$ and $B$ are finalized, contradicting induction hypothesis \ref{non-adjacent}.

The third bullet could become violated as a result of $s$ if either $W=A$ or $Z=A$.  We consider the two cases in turn.
To derive a contradiction, suppose the third bullet is true with $W=A$ for some reachable node $X$ in $C_i$.
Then $Z=A\rightarrow right = B$.  Since $s$ is performed by a splice($A,B,C$) operation, $B\rightarrow right = C$ by induction hypothesis \ref{pending-splice}, so $X=C$.
Thus, $C\rightarrow priority = X\rightarrow priority > W\rightarrow priority = A\rightarrow priority$.
This contradicts the fact that the test at line \ref{priority-switch} of splice($A,B,C$) returned true
so that $s$ could be performed.
Next, to derive a contradiction, suppose the third bullet is true with $Z=A$.
Then, $A$ is finalized in $C_i$.
Since $s$ is performed by a splice $(A,B,C)$, $B\rightarrow left = A$, by induction hypothesis \ref{pending-splice} and $B$ is also finalized in $C_i$.  This contradicts induction hypothesis \ref{non-adjacent}.

To show that $s$ preserves claim \ref{pending-splice}, it is sufficient to show that there is no splice($*,A,B$) operation in progress at $C_i$.
To derive a contradiction, suppose there is such a pending splice.
By the test on line \ref{test-priority}, $A\rightarrow priority < B\rightarrow priority$.
Since $s$ is performed by a splice($A,B,C$) operation, we similarly have that $A\rightarrow priority > B\rightarrow priority$, a contradiction.

To show that $s$ preserves claim \ref{still-reachable}, observe that the only node that could become unreachable as a result of $s$ is $B$, and $B$ is finalized by line \ref{finalize-cas} prior to $s$.


\bigskip
{\bf Case 3}:  $s$ is a successful CAS on line \ref{left-cas1} that changes $Y\rightarrow left$ from $X$ to $W$.

The proofs that claims \ref{non-adjacent}, \ref{priorities}, \ref{pending-splice} and \ref{still-reachable} are preserved by $s$ are symmetric to the proofs of these claims given in Case 2.

\Eric{Still have to fill in the proofs of the other two claims, which might differ slightly from Case 2, but they should be very similar.}

\bigskip
{\bf Case 4 and 5}:  $s$ is a CAS on line \ref{left-cas2} or \ref{right-cas2}.  These arguments are symmetric to Cases 2 and 3, respectively.

\end{proof}




==> proof.tex <==
% !TEX root =  main.tex

\section{Proof of Correctness of the List (some old, rough notes)}

It seems to me that remove and remove-rec are part of the client that uses this list data structure, not part of the list data structure itself, so the proof of linearizability of the list should just focus on 
linearizing operations splice (3 varieties), readRight, getHead (which returns the head node of the list) and prepend (which adds a node to the head of the list), since these are the only operations needed by our application.


Invariant 1 (no two finalized nodes in a row):  If $x.status = finalized$ then ($x.left = nil$ or $x.left.status \neq finalized$) and ($x.right = nil$ or $x.right.status \neq finalized$).

The proof of Inv 1 might have to be rolled up with proving that left and right pointers of a node do not change after it is finalized.

Define $x.absRight$ to be the first non-finalized node reached by following right pointers from node $x$ (or nil if no such node exists).
Define $x.absLeft$ similarly.

Then, proving linearizability just needs the following 3 claims.

Claim 1:  The abstract pointers form a doubly-linked list (which we call the abstract list).
[In other words, if x is not finalized, $x.absRight.absLeft = x$ and $x.absLeft.absRight = x$,
and it's trivial to see there are no cycles in the abstract list, since version numbers of nodes are in order.]
This abstract list changes only at the linearization point of a splice (which removes a single node from the abstract list) and prepend (which adds a node to the head of the abstract list).

Proof sketch for Claim 1:
\begin{itemize}
\item 
It's pretty obvious that the CAS that finalizes a node preserves the doubly-linked list structure of the abstract list, and that it removes the newly-finalized node from the abstract list.
\item
Will have to prove this for the prepend operation (not yet written).  Actually, there might be a slight hiccup here; the invariant described in Claim 1 might be temporarily violated right at the head of the list during a prepend.
\item
The only other steps that could modify the abstract list are the CAS steps on left and right pointers in splice, readRight and readLeft.  We just have to prove that when $x.right$ is changed from $y$ to $z$, $y$ is already finalized and $y.right = z$. This will probably make use of Invariant 1.
\end{itemize}

Claim 2:  At the linearization point of a $readRight(x)$ operation that returns $y$, $x.absRight=y$.

The proof of Claim 2 should be easy using Invariant 1.  (May need a precondition that $x$ is not finalized when we call $readRight(x)$.)  But what happens if the application calls readRight on a node that has been finalized by a concurrent operation?

Claim 3:  At the linearization point of a $getHead$ operation that returns $x$, $x$ is the first node of the abstract list. 

Proof of Claim 3 should be fairly trivial, since we never finalize the head of the list, so Head should always point to the first element of the abstract list.

==> step3-old.tex <==
% !TEX root =  main.tex


\section{Reclaiming Memory from the Multiversion Data Structure \Hao{this section is in the process of being split.}}

\Eric{Change depreciate to deprecate throughout this file}

Starting with a basic concurrent data structure, Wei et al.~\cite{WBBFRS21a} describe how to transform it using
multiversioning to support
complex query operations.
A query operation takes a snapshot by reading a global timestamp, and then traverses the version
of the data structure corresponding to that timestamp to determine the result of the query.
Here, we describe how to combine the algorithms described in the previous sections
to handle memory management of this augmented multi-versioned data structure.
We call operations on the basic data structure {\it frontier operations},
because they take place on the current version. The operations working on the snapshot of the
data structure are called \emph{snapshot operations}. \Yihan{I added the definition for snapshot operation because we seem to use it below.}

We assume that the basic data structure comes with a memory reclamation scheme.  In this section, we show how to extend this scheme to the snapshottable version of the data structure.
We make no assumptions about the original memory reclamation scheme
%\footnote{The original scheme, for example, could use hazard-pointers, epoch, or reference-counting based collection techniques.}
except that it calls \op{retire} on a node when it becomes unreachable from the roots of the data structure and \op{free} on a node when it is safe to collect.
Operations invoked after a node is retired cannot possibly reach the node, but operations
that were in progress when it was retired might
still access it.  A node is freed when it is impossible for any operation to access it.
Many existing memory reclamation schemes, including hazard-pointers~\cite{}, hazard-eras~\cite{}, or epoch based collection~\cite{}, fit into this framework.
\Eric{Citations missing}

\Hao{The snapshot transformation from our PPoPP paper does not change the original data structure's memory reclamation scheme.}

There are three types of objects in the snapshottable version of the data structure: nodes and objects used by the original data structure (which we will broadly refer to as \dnode{}s), version list nodes (\vnode{}s), and Descriptor objects used by our \op{remove} operation.

A \dnode{} can be reclaimed when neither frontier nor snapshot operations need it any longer.
When the original data structure's memory reclamation scheme \op{frees} a node,
we know that it will not be needed by any frontier operation,
so we just need to track which \dnode s are needed by the snapshot operations.
This is done by tagging each \dnode{} with a birth and retire timestamp.
After a \dnode\ is allocated \Eric{but before it is attached to the data structure?},
its birth timestamp is set by reading the Camera
object's timestamp field and writing it into the appropriate field of the \dnode{}
(this is done by calling \op{setBirthTimestamp} from Figure \ref{fig:step3-dnode}).
Similarly, a \dnode's retire timestamp is set when the original data structure's
memory reclamation scheme calls \op{retire} on the node. A \dnode{} is not
needed by any snapshot operation if there is no announced timestamp  between
its birth timestamp (inclusive) and retire timestamp (exclusive).
We track this using the \rangetracker{} data structure from Section \ref{sec:identify}.
The instance of the \rangetracker{} data structure for
\dnode{}s is separate from the one for \vnode{}s.
Whenever the original data structure's memory
reclamation scheme \op{frees} a \dnode{},
we instead add this node to the \dnode\ range tracker.
When a \dnode{} gets returned by the range tracker,
we first call \op{remove} on the \vnode\ at the head of any
version lists pointed to by the \dnode{} and then free the \dnode{}.
The call to \co{remove} is important because without it, the heads of the version
lists would never be collected. \dnode{}s returned by the range tracker are
safe to free because they are not needed by any frontier or snapshot operation.
These steps are shown in \op{freeDNode} operation in Figure \ref{fig:step3-dnode}.
%Note that there could still be \vnode{}s pointing to the \dnode{}, however none of those pointers will be traversed.
\Hao{argue for space and time bounds}.

The reclamation of \vnode{}s and Descriptor objects is managed using
concurrent reference counting. To maintain our desired time and space bounds,
we use an existing solution for concurrent reference counting as a black box~\cite{BW20b}.
This implementation of reference counting has \Eric{expected?} constant-time overhead and guarantees
that there at most $O(P^2)$ delayed decrements.
A decrement is considered to be delayed if a reference counted pointer
has been swung away from a node and its reference count has not yet been decremented.
A node is collected as soon as its reference count hits 0.
Using existing implementations of concurrent reference counting 
\Eric{Do you mean "Using the reference counting scheme of \cite{BW20b}"}
requires
extending each \vnode{} and Descriptor object with an extra field to store
its reference count and replacing raw pointers to \vnode{} and Descriptor
objects with reference-counted pointers (\rcptr{}) and
atomic-reference-counted pointers (\arcptr{}),
which automatically manage the reference counts of the objects they point to.
Both \rcptr{} and \arcptr{} support all the standard operations that raw pointers support.
\Eric{Does this just mean reads and writes?  If so, I would say \rcptr\ supports reads and writes, while \arcptr supports CAS in addition.}
Collecting an object clears all the reference counted pointers in that object,
which could result in recursive collection.
%The difference between \rcptr{} and \arcptr{} is that
An \arcptr{} supports CAS and is more \Eric{What does more mean?} concurrency safe,
whereas an \rcptr{} only supports read and write and is safe if
reads do not race with writes.
Operations on \arcptr{}s are allowed to arbitrarily race with one another.
In Algorithms \ref{fig:list-alg-full-gc} and \ref{fig:vcas-alg-youla-gc},
we use \arcptr{}s to store the left and right pointers
as well as the left and right Descriptor pointers of each \vnode{}.
We also use an \arcptr{} to store the head of each version list.
We use \rcptr{}s for local pointers. We also use \rcptr{}s for the VNode pointers
in each Descriptor object because these pointers are written once,
before any other process has access to it, so there are no read-write races on the pointers.

In Algorithm \ref{fig:vcas-alg-youla-gc},
the RangeTracker stores raw pointers rather than reference counted pointers.
\Eric{Say whether you are talking about the the range tracker for Dnodes or the one for Vnodes?  Pointers to what?  Dnodes?  Vnodes?  Why is this okay?
I.e., why doesn't it cause problems with the reference counting?}
This simplifies our space bound arguments because it reduces the number of
reference counted pointers we have to reason about.
% because we only have to count the number of VNodes held by pointers in Figures \ref{fig:vcas-alg-youla-gc} and \ref{fig:list-alg-full-gc}.
When a raw pointer gets returned from the range tracker data structure, it is safe
\Eric{What is the criterion for such a conversion to be safe?}
to convert it into a reference counted pointer
(Line \ref{line:to-rc-ptr} of Figure \ref{fig:vcas-alg-youla-gc})
because the VNode it points to is still reachable
(\Hao{according to the definition from Step 2}) and definitely not collected.

A limitation of reference counting garbage collection is that
%a node can be collected only when it is not part of any cycle.
cycles must be broken before a node can be collected.
While there are cycles in our
version lists, we can show that \vnode s that have been spliced out are not part of
any cycle (with the exception of a few \vnode s
that are temporarily still pointed to by Descriptors).
This is because \vnode s reachable from a spliced out \vnode\ $n$ were either spliced
out after $n$ or not yet spliced out. Therefore, spliced out \vnode s
cannot be part of any cycle.
\Hao{Add some more explanation here.}

\Hao{At the beginning, say it is a small change, then at the end, say without this change, the space bounds would not hold.}
To get good overall bounds on the number of \vnode{}s, we need to modify
our linked list algorithm slightly (from Section \ref{sec:vlists}).
The changes are shown in blue in Figures \ref{fig:list-alg-full-gc}
and \ref{fig:vcas-alg-youla-gc}. Our goal is to bound the number of \vnode{}s
that have been spliced out of a version list but not collected.
Without these changes, this bound could be high, because a large number of
spliced out nodes could be kept alive by a slow process that paused on a single \vnode{}.
\Eric{Maybe explain how this could happen}
To prevent this, we modify the algorithm so that spliced out \vnode{}s
only point to ancestors in the implicit tree.
Therefore each \vnode{} that has been spliced out but not yet
collected can only keep alive at most $O(\log L)$ other spliced out \vnode{}s.
To achieve this property, after splicing out a node, we set its left and right
pointers to $\top$ if they point to descendants in the implicit tree.
This requires changing how we traverse version lists. Whenever a node with
left pointer $\top$ is encountered, the traversal moves right instead
(see \op{readVersion} from Figure \ref{fig:vcas-alg-youla-gc}).
The left and right pointers of a node cannot both be $\top$ because whenever
\op{splice(A, B, C)} is called, it is guaranteed that either \A\ or \C\ is an ancestor of \B.
This new traversal algorithm can be viewed as switching between two phases,
a forward traversal phase and an upward traversal phase.
If the \vnode{} the traversal is currently on has not been spliced out,
then it performs a forward traversal. If it has been spliced out,
then it performs an upward traversal in the implicit tree.
We show that upward traversals during a search all have distinct source nodes,
while forward traversals during a search all have distinct destination nodes.  \Hao{Formally proven below}
%We show that whenever an upwards traversal is performed from \A\ to \B,
%the source nodes are distinct and whenever a forward traversal is performed from \A\ to \B,
%the destination nodes are distinct.
This means that these modification do not affect the time complexity of the traversal algorithm.
\Eric{Explain}

\Eric{Once you introduce right traversals, you could also (in principle) traverse into parts of the list that were added by tryAppend operations after you started the traversal, raising the danger of the search running forever.}

\Eric{We also need to explain why the traversal finds the right node to return}

% \Hao{the new algorithm for step 3 does not require nodes to be finalized.}
% \Eric{Let's ignore this, and still do the finalize step}

In addition to modifying the traversal algorithm, we need to check that none of the other version list operations are affected by our change which sets some pointers to $\top$ after a splice. This involves checking all the read and CAS operation in Figure \ref{fig:list-alg-full-gc} to make sure they still behave correctly and these checks are performed in the proof of Lemma \ref{lem:remove-with-gc}. Intuitively, we will show that whenever a process reads $\top$ from a left or right pointer of a node $N$, it will never use the value it read because $N$ has already been spliced out.


To bound the number of \vnode{}s that have been spliced out, but not freed, consider all the possible reference counted pointers to these nodes. They can be pointed to by:

\begin{itemize}
	\item local pointers held during vCAS, vRead, readVersion, remove, and tryAppend operations
	\item pointers from the left/right pointers of other \vnode{}s
	\item the head pointer of a version list
	\item pointers from Descriptors
\end{itemize}

There could also be pointers from the range tracker data structure, but these are not reference counted, so we do not need to worry about them when counting space complexity. \Hao{add more explanation, we don't need to reference count them, and this is why they don't count towards space complexity.}
%Our goal is to bound the number of spliced out \vnode{}s that are still pointed to.
%We classify pointers to spliced out \vnode{}s into three disjoint categories, internal pointers, deep external pointers, and shallow external pointers. Internal pointers are pointers from one \vnode{} to another. All other pointers are considered external pointers. An external pointer to a node $n$ is considered to be shallow if $n$'s left and right neighbours have not been spliced out. A deep external pointer could prevent the collection of $O(\log L)$ \vnode{}s (where $L$ is length of a version list \Hao{needs to be defined more precisely}) due to internal pointers, where as a shallow external pointer does not prevent the collection of any other \vnode{}. If $D$ and $S$ represent the number of deep and shallow external pointers, the number of spliced out \vnode{}s that have a reference counted pointer to it is at most $O(D\log{} L + S)$ (this is proven in Lemma \ref{lem:ref-count}). The reference counting algorithm we use ensures that all of the ones that are not pointed to have already been collected, except for a set of at most $O(P^2)$ due to the $O(P^2)$ differed decrements.
%We will show that $D \in O(P^2)$ and $S \in O(L_t + P^2)$, where $L_t$ is the total length of all the version lists (number of reachable nodes, using the notion of reachable defined in Step 2).
%Since there are $O(L_t + P)$ \vnode{}s that have been allocated, but not spliced out, the total number of \vnode{}s that have been allocated and not freed is $O(L_t + P^2 \log{} L)$.

\Hao{Make Figure 7 consistent with the earlier version of the figure.}

\Hao{Talk about how using reference counting would changes these operations to be amortized constant time. Maybe there are ways to deamortize this.}

\Hao{We talked about replacing the step 2 version of the algorithm with the step 3 version. I think it might be still nice to show the step 2 version because it could be of independent interest. Someone may wish to use step 2 with a different memory management scheme. In which case following right pointers doesn't really make sense.}
\Eric{I agree; the original algorithm is complicated enough, so it is good to do the modifications in a separate figure (which will be beyond the 15-page limit)}

\subsection{Traversing to the right of the starting node}

\Hao{This section is mostly notes/ideas and is not intended to be part of the final submission.}

In a previous comment, Eric brought up the issue that the traversal in a \op{readVersion} operation might actually visit parts of the list that were newly added by \op{tryAppend} operations.
This looks to be a real issue that would increase the time complexity of \op{readVersion} operations.
In our PPoPP paper, the complexity of \op{readVersion(ts)} was proportional to the number of \op{vCAS} instructions between the \op{takeSnapshot} returning \op{ts} and the start of the \op{readVersion(ts)}.
Due to the issue of visiting newly added nodes, if we do not modify the current algorithm at all, the amortized bounds for \op{readVersion(ts)} in step 3 would have an extra additive $O(\log L)$ term compared to the bounds from the PPoPP paper.
A more detailed description of why this is the case will appear below.
Each multi-point query might call \op{readVersion} multiple times and each call might experience this additive $O(\log L)$ overhead, so the overhead sounds very significant.
However, in our PPoPP paper, we usually state the complexity of multi-point queries as its sequential cost plus the number of update instructions concurrent with it.
This bound would still hold even with the extra overhead per \op{readVersion} because in order for a \op{readVersion} to experience $\log L$ overhead, it would have to be concurrent with $L$ \op{vCAS} instructions.
Perhaps we are happy enough with these bounds, in which case we do not need to modify our current algorithm.

This section will start by justifying some of the claims in the previous paragraph and showing an execution where the issue of traversing newly added nodes occurs. \Hao{TODO: complete section}

Currently, the only solution to this problem that I'm aware of is to prevent a node's left pointer from being set to $\top$ if it is the starting point of some \op{readVersion} operation. I believe this is possible, but unfortunately, this solutions seems very complicated to implement.

\subsection{Proof of Space Bounds}

\subsubsection{Bounding the number of \dnode{}s}

\Hao{We probably also need a theorem stating that our reclamation technique for \dnode{}s takes constant time.}

\Eric{Following theorem uses $H_{max}$ to denote something a little different from the $H_{max}$ used in Step 1.} 

\begin{theorem}
\label{thm:dnode-space}
	We consider a \dnode{} to be \emph{necessary} if it is either not freed by the original data structure's memory reclamation scheme or if there exists an announced timestamp in between its birth and retire epoch.
	Let $D_{max}$ be the maximum number, over all configurations in the execution, of the number of necessary \dnode{}s.
	In any configuration, there are $O(D_{max} + P^2 \log P)$ \dnode{}s that have been allocated but not freed.
	\Hao{make this theorem statement more precise.}
\end{theorem}

\begin{proof}
	We begin by noting that a \dnode{} is depreciated as soon as it is freed by the original data structure's memory reclamation scheme.
	The set of \dnode{}s that have been allocated but not freed can be partitioned into three set, one set $A$ for \dnode{}s that have not been freed by the original data structure's memory reclamation scheme, another set $B$ for \dnode{}s that have been passed to \op{depreciate} but not returned, and another set $C$ for \dnode{}s that have been returned by some \op{depreciate} but not freed.
	Since any \dnode{} that is not yet depreciated is necessary, $|A| < D_{max}$.
	The nodes returned by \op{depreciate} are freed before the next call to \op{depreciate} by the same process, so by Lemma \ref{lem:deprecateRetVal}, each process contributes at most $4 P \log P$ nodes to the set $C$, so $|C| \leq 4P^2 \log P$.
	
	To complete the proof, it remains to bound $|B|$.
	Recall that a depreciated object is said to be \emph{needed} if its interval contains an active announcement.
	This means that all needed depreciated \vnode{}s are also necessary.
	Therefore $D_{max}$ is an upper bound on the number of needed depreciated \vnode{}s across all configurations of the execution.
	By Theorem \ref{step1-space}, $|B| \leq 2D_{max} + 25 P^2\log P$, which completes the proof.
\end{proof}

\subsubsection{Bounding the number of \vnode{}s and Descriptor objects}

\begin{theorem}
	\label{thm:step3-vnode-space}
	Overall, there are at most $O(T + P^2 \log{} L)$ \vnode{}s and $O(T + P^2)$ Descriptor objects, where $L$ is the maximum number of successful \op{tryAppend}s on a single version list and $T$ is the total number of \lrreachable{} nodes across all the version lists.
\end{theorem}

\begin{proof}
	
\begin{itemize}
	\item Note: Throughout this proof, node always refers to \vnode{}.
	\item Definition: \lrunreachable{} node (\Hao{perhaps pick better names. This one stands for left-right-unreachable}): A \vnode{} that is has been allocated and not deallocated and not reachable according to the definition in Step 2. A \vnode{} is also considered \lrunreachable{} before it is appended.
	\item Our goal is to bound the number of \lrunreachable{} \vnode{}s.
%	\item Definition: A spliced out \vnode{} is a \vnode{} that has been made \lrunreachable{} due to a splice.
	\item Definition: An \downptr{} is a pointer from one node to another such that the destination node is a descendant of the source.
	\item Definition: An \upptr{} is a pointer from one node to another such that the destination node is a ancestor of the source.  \Eric{Maybe up-pointer and down-pointer would be easier to remember, because it might be hard to remember whether ancestor-pointer means the pointer is in the ancestor or to the ancestor} \Hao{I'm ok with this new terminology.}
	\item Observation: Whenever a node A points to a node B, both A and B's priority have already been set and their priorities cannot be equal. This is because a node's priority is set before it points to anything and before any node can point to it.
	\item Definition: A \srcnode{} (\Hao{pick a better name for this}) is an \lrunreachable{} node that is not pointed to by any \upptr{}s.
	\item Claim: All \lrunreachable{} nodes are reachable by following \upptr{}s starting from a \srcnode{}. \Hao{I believe this just involves proving that \upptr{}s do not form a cycle and showing that all non-source \lrunreachable{} nodes are pointed to by an ancestor pointer from a \lrunreachable{} node.}
	\item \Hao{bound the number of version lists for which the head node has been removed, but the head pointer has not been cleaned up.}
%	\Eric{Bad notation:  $L$ and $L_t$ seem to count unrelated notions}
%	\Hao{Changed $L_t$ to just $T$.}
	\item Claim: There are at most $O(T + P^2)$ Descriptors that have been allocated but not freed. This is because there are $O(P)$ Descriptors pointed to by local pointers, $O(T)$ pointed to by \lrreachable{} nodes (\lrunreachable{} do not point to any valid Descriptor objects), and $O(P^2)$ Descriptors that have no pointers to them, but have also not been freed.
	\item Claim: There are at most $O(L_t + P^2)$ \srcnode{}s. A source node is either pointed to by (1) a Descriptor object, (2) a local pointer, (3) no pointers, and (4) a \downptr{}. There are at most $O(L_t + P^2)$ \srcnode{}s of type (1), $O(P)$ of type (2), $O(P^2)$ of type (3), $O(P)$ of type (4). To show the bounds for type (4), there are only two ways for a \lrunreachable{} node to be pointed to by an \downptr{}. First, it could be that the node pointing to it has been spliced out and its left/right pointer has not yet been set to $\top$. Second, it could be that the node pointing to it was newly allocated for a \op{tryAppend} that is now guaranteed to fail. There can only be a constant number of such cases per process.
	\item Claim: From each \srcnode{}, there are at most $O(\log{} L)$ nodes reachable by following \upptr{}s. This is because all the reachable nodes are ancestors of the \srcnode{}. However, some of these $O(\log{} L)$ may be \lrreachable{}, so we don't want to count these.
	\item Claim: It turns out that whenever a \srcnode{} $n$ is pointed to by a Descriptor installed in a \vnode{}, all of the $O(\log{} L)$ nodes reachable from $n$ by following \upptr{}s are \lrreachable{}. \Hao{this requires a proof, perhaps we can reuse some lemmas from step 2}
	\item Claim: There are $O(P^2)$ \srcnode{}s that are not pointed to by a Descriptor installed in a \vnode{}, and from each node $n$ in this set, there could be $O(\log{} L)$ \lrunreachable{} nodes that are reachable from $n$ by following \upptr{}s. Therefore, the number of \lrunreachable{} nodes is bounded by $O(L_t + P^2 \log{} L)$.
	\item Summary: Overall, there are at most $O(L_t + P^2 \log{} L)$ \vnode{}s and $O(L_t + P^2)$ Descriptor objects.
\end{itemize}
	
\end{proof}

\subsubsection{Overall Space Bounds}

We say that a \vnode{} is \emph{necessary} if it is pointed to by a \dnode{} that has not yet been depreciated (i.e. freed by the original data structure's memory reclamation scheme) or if its interval \Hao{define more formally} contains an announced timestamp \Hao{also define more formally}.
Let $D_{max}$ and $V_{max}$ be the maximum number of necessary \dnode{}s and \vnode{}s throughout a history.

\begin{theorem}
\label{thm:overall-space}
	The overall space usage of a snapshottable data structure (using VersionedCAS objects implemented with steps 1-3 \Hao{make this statement more precise}) is $O(D_{max} + V_{max} + P^2 \log P + P^2 \log L)$, where $L$ is the number of successful \op{tryAppend} operations.
\end{theorem}

\begin{proof}
	We first bound the number of \vnode{}s that are allocated, but not depreciated.
	Let $b$ be the maximum number of versioned CAS objects in each \dnode{}.
	We can partition \vnode{}s into two sets: a set $A$ of \vnode{}s that are at the head of some version lists and a set $B$ of \vnode{}s that are not at the head of any version list.
	The size of $A$ is bounded by the number of \dnode{}s that have not been freed times $b$.
	Assuming $b$ is a constant \Hao{are we ok with this assumption?}, $|A| \in O(D_{max})$.
	%When $b$ is not a constant, I guess the \dnode{}s would have to be very large, so the space probably amortizes out.
	Other than the head of each version list (and \vnode{}s that have been allocated, but not yet appended), all over \vnode{}s have been depreciated.
	The set of needed depreciated \vnode{}s is a subset of the necessary \vnode{}s, so by Theorem \ref{step1-space}, the number of depreciated objects that have not yet been returned is at most $2V_{max} + 25 P^2 \log P$.
	By Lemma \ref{lem:deprecateRetVal}, each call to \op{depreciate} returns at most $4P \log P$ objects, so there are at most $4P^2 \log P$ that have been returned but not passed to \op{remove}.
	Let $H$ be the set of \vnode{}s that were added by a successful \op{tryAppend} and not yet passed to \op{remove}.
	Every \vnode{} in $H$ is at the head of a version list (which means they are pointed to by some \dnode{}) except for a set of size $P$.
	Therefore $H \leq V_{max} + P$.
	By Proposition \ref{space-bound}, the number of \vnode{}s that have been passed to \op{remove} and are still \lrreachable{} is $O(H + P \log L)$, where $L$ is the number of successful \op{tryAppend} operations.
	The total number of \lrreachable{} \vnode{}s (also counting those that have not been passed to \op{remove}) is also $O(H + P \log L)$.
	By Theorem \ref{thm:step3-vnode-space}, the number of \vnode{}s that are \lrunreachable{}, but not yet freed is $O(H + P^2 \log{} L)$.
	Therefore the overall number of \vnode{}s that have been allocated but not freed can be computed as follows:
	\begin{itemize}
		\item $O(P)$ \vnode{}s that have been allocated, but not yet appended,
		\item $O(D_{max})$ that have been appended and are still at the head of the version list,
		\item $O(P)$ that have been replaced as the head of the version list but are not yet depreciated,
		\item $O(V_{max} + P^2 \log P)$ that have been depreciated, but not yet returned,
		\item $O(P^2 \log P)$ that have been returned, but not yet passed to remove,
		\item $O(H + P \log L)$ that have been removed, but are still reachable
		\item $O(H + P^2 \log L)$ that are unreachable, but not yet freed.
	\end{itemize}	
	
	Since $H \leq V_{max} + P$, the total number of \vnode{}s that have been allocated but not freed is $O(D_{max} + V_{max} + P^2 \log P + P^2 \log L)$.
	
	By Theorem \ref{thm:step3-vnode-space}, the total number of descriptor objects is in $O(H + P^2 \log{} L) \subset O(V_{max} + P^2 \log{} L)$, and by Theorem \ref{thm:dnode-space}, the total number of \dnode{}s is $O(H_{max} + P^2 \log P)$.
	Assuming all these objects take constant space, the overall space usage is $O(D_{max} + V_{max} + P^2 \log P + P^2 \log L)$.
\end{proof}

\subsection{Proof of Correctness}

\begin{lemma}
\label{lem:step3-safety}
	Our memory management scheme is safe, meaning that an object will never be accessed after it is freed.
\end{lemma}

\begin{proof}
	Our algorithm explicitly frees memory for three types of objects: \vnode{}s, \dnode{}s, and descriptor objects.
	Descriptor objects and \vnode{}s are freed by the concurrent reference scheme when there are no more reference counted pointers to these objects and \dnode{}s are freed on Line \ref{} of Figure \ref{fig:step3-dnode}.
	
	We first argue that whenever a Descriptor or \vnode{} is freed, there are no more references to that object, which implies that there cannot be any future accesses to that object.
	This is easy to show for Descriptor objects because every reference to a Descriptor object is reference counted.
	In the case of \vnode{}s, most pointers are reference counted except for those stored in the range tracker data structure (which are just raw pointers).
	Note that in our algorithm, we never dereference these raw pointers, so the only potentially dangerous operation is the conversion from raw pointers to reference counted pointers on Line \ref{}.
	This conversion is safe as long as the reference count . \Hao{I don't know if we need to prove this.}
	
	
	The range tracker data structure never dereference any of these raw pointers, but after \op{depreciate} operation returns a list of raw pointers on Line \ref{} of Figure \ref{}, these pointers are dereferenced on Line \ref{} when they are converted into
	We will argue that
	
	
\end{proof}

%\begin{lemma}
%	\label{lem:timestamp}
%	If the timestamps of $A$ and $B$ are both valid and either $A \rightarrow B$ or $A \leftarrow B$, then $A$'s timestamp is at most $B$'s timestamp. \Hao{I'm not sure if we need this lemma anymore.}
%\end{lemma}

\Hao{Change all time bounds to expected time.}

% \begin{proof}
% 	By Lemma \ref{}, if $A \rightarrow B$ or $A \leftarrow B$ then $A <_c B$.
% 	Increasing counter value implies appended later, so $B$ was appended later than $A$.
% 	By Lemma \ref{} from the PPoPP paper, ..
% 	Therefore $B$ was a
% \end{proof}

\begin{lemma}
\label{lem:traversal-correctness}
	Figure \ref{fig:vcas-alg-youla-gc} shows a linearizable implementation of a \op{VersionedCAS} object.
	\Hao{This lemma is mostly used to argue that the \op{readVersion} behaves correctly. This requires the assumption that \op{readVersion} is not run on a version list after its head has been removed.}
\end{lemma}

\Hao{Define a separate find function.}

\begin{proof}
	
\end{proof}

\Hao{I'm not sure where to place this section because Lemma \ref{lem:step3-safety} is required for Lemma \ref{lem:remove-with-gc}, but Lemma \ref{lem:remove-with-gc} is required for Lemma \ref{lem:traversal-correctness}. Perhaps the proof of time and correctness should be combined.}

\subsection{Proof of time bounds}

%
%In Section \ref{}, we've already shown that ...

The goal of this section is to show that steps 1, 2 and 3 combined add only constant time overhead to the versioned CAS objects implemented by Wei et al.~\cite{WBBFRS21a}. More precisely, we would like to show that the time complexities of \op{readVersion} and \op{vRead} are maintained up to a constant factor and that \op{vCAS} takes amortized constant time (i.e. $M$ \op{vCAS} operations take time $O(M)$ in total).

There are several components to this proof:
\begin{itemize}
	\item need to show that reference counting operations take amortized constant time. (Lemma~\ref{lem:ref-count})
	\item Then we need to consider calls to \op{depreciate} and \op{remove} that were added to \op{vCAS}. (Observation~\ref{obs:depreciate-remove})
	\item We also need to show that the changes to \op{remove} do not affect its constant time bounds. (Lemma~\ref{lem:remove-with-gc})
	\item Finally, we need to show that \op{readVersion} does not go back to the same node multiple times. (Lemma~\ref{lem:traversal})
\end{itemize}

\Eric{In following lemma, we assume constant time allocation.  Should we instead cite DISC 2020 paper or \cite{BW20b}?}

\begin{lemma}
\label{lem:ref-count}
	Read-only operations on \rcptr{} and \arcptr{} (including reading and dereferencing) all take constant time. Assuming that memory can be allocated and de-allocated in constant time and assuming that each object contains a constant number of reference counted pointers, write operations on \rcptr{} and \arcptr{} (including store, CAS and destruct) take amortized constant time meaning that $M$ write operations take $O(M)$ time in total.
\end{lemma}

\begin{proof}
	Theorem X from~\cite{} states that read-only operations take constant time, and that write operations, ignoring the call to \op{delete}, take constant time as well.
	So it suffices to argue that the cost of \op{delete} can be amortized to earlier write operations.
	When the \op{delete} operation is called on an object, for each reference counted pointer $ptr$ that belongs to the object, \op{delete} decrements the reference count of the object pointed to by $ptr$.
	If an object's reference count hits 0, then \op{delete} is recursively called on that object.
	Since each object contains a constant number of reference counted pointers, the time complexity of a \op{delete} operation is proportional to the number of reference counts decremented by the \op{delete}.
	We can amortize these reference count decrements as follows. Suppose the delete operation decrements the reference count of object $Y$ because it was pointed to by field $F$ of object $X$. We charge the cost of this decrement to the write operation that caused $X.F$ to point to $Y$.
	In this way, we guarantee that each write operation is charged with at most one decrement from a \op{delete} operation.
	Therefore, each write operation on a reference counted pointer takes amortized constant time.
\end{proof}

The following lemma proves both the correctness of the \op{remove} algorithm in Figure~\ref{fig:list-alg-full-gc} as well as its time bounds.
It's convenient to combine these two arguments because they both boil down to arguing that the \op{remove} algorithm in step 3 behaves the same way as in step 2.
In terms of time bounds, we will show that $R$ remove operations takes $O(R)$ time.

\begin{lemma}
\label{lem:remove-with-gc}
	Proposition~\ref{space-bound} holds for the \op{remove} algorithm in Figure~\ref{fig:list-alg-full-gc}. Furthermore, \op{tryAppend} takes constant time plus the cost of $O(1)$ operations on reference counted pointers. Similar to Proposition~\ref{remove-amortized-time}, $R$ \op{remove} operations take $O(R)$ time plus the cost of $O(R)$ operations on reference counted pointers.
%	Both Propositions~\ref{remove-amortized-time} (I believe this proposition should also state the time complexity of tryAppend) and~\ref{space-bound} hold for the \op{remove} algorithm in Figure~\ref{fig:list-alg-full-gc}. Propositions~\ref{space-bound} would have to be slightly modified to say that
\end{lemma}

\begin{proof}
	We begin by comparing Figure~\ref{fig:list-alg-full-gc} with Figure~\ref{fig:list-alg-full} and arguing that the changes made in Figure~\ref{fig:list-alg-full-gc} do not affect the behavior of the original algorithm.
	First, let's consider the changes highlighted in blue in isolation (i.e. replacing all reference counted pointers in Figure~\ref{fig:list-alg-full-gc} with raw pointers).
	The major change is Lines \ref{clear-left-gc} to \ref{clear-right-gc} of \op{splice}, which set the left and right pointers of the spliced out node to $\top$ if they point to descendants, as well as the additional if statement on Line \ref{check-top-gc}.
	This change only adds constant time overhead to \op{splice} and \op{tryAppend}, but we need to argue that it does not change the time complexity and correctness of other parts of \op{remove} or \op{tryAppend}.
	To do this, we need to go through every read and CAS on left/right pointers that could have potentially seen the value $\top$ and argue that the operation would have behaved the same way had it seen the value that was overwritten by $\top$.
	
	We begin by reasoning about CAS operations. By Invariant \ref{inv}.\ref{splice-args}, we know that in the \op{remove} algorithm from Step 2, after \op{splice(*, B, *)} is called on a node, CAS operations on the left and right pointers of \op{B} can never succeed. \Hao{also need to argue that there is no CAS operation with the same new and expected value.}
	% argument draft:
%	CAS operations on left and right pointers come from just two methods \op{splice} and \op{tryAppend}.
%	By Lemma \ref{}, we know that whenever \op{splice(A, B, C)} is called on a node, the input parameters are distinct, which means the new and expected values of the CAS it performs is never the same.
%   Similarly, the parameters passed to \op{tryAppend} are always distinct, so none of the CASes it performs has the same new and expected value.
	Therefore setting \op{B}'s left or right pointer to $\top$ during a \op{splice(*, B, *)} does not impact the return value of any other CAS operation.
	
	Consider the reads on lines \ref{read-left} and \ref{read-right}. We check if $B$ is finalized immediately after the two reads. If either of them were $\top$, then the check will fail, so the operation returns without making use of the invalid pointer.
	
	Consider the read of \op{C->left} on line \ref{sur-test-???-gc}. If the read of \op{C->left} returns $\top$, then $C$ was marked and frozen, so even if the previous value of \op{C->left} was equal to $B$, the \op{spliceUnmarkedRight} would have returned false anyways after failing the next CAS on Line \ref{store-left-desc-gc}.
	Therefore the return value, behavior, and time complexity of \op{spliceUnmarkedRight}, does not change. The same argument applies to the read of \op{A->right} in \op{spliceUnmarkedLeft}.
	
	For the read on line \ref{test-right-gc}, if $A$ is finalized, then $B$ must be \lrunreachable{} \Hao{need to verify the previous claim. A lemma from step 2 might be helpful here.}, so if \op{A->right} equals $\top$, then line \ref{test-right-gc} returns false as desired (since the CAS operations on Lines \ref{left-cas-gc} and \ref{right-cas-gc} are guaranteed to fail).
	This does not affect the time complexity of \op{splice}.
	
	For the read on Line \ref{mr-read-left-gc}, if \op{B->left} is $\top$, then $B$ has already been finalized, so a newer node has already been installed, in this case the \op{tryAppend} is guaranteed to fail and it will return false on Line \ref{check-top-gc}. Conversely, if \op{tryAppend} returns false on Line \ref{check-top-gc}, then $B$ is no longer at the head of the version list so the CAS on Line \ref{head-cas-gc} is guaranteed to fail.
	
	Therefore, adding Lines \ref{clear-left-gc}-\ref{clear-right-gc} and \ref{check-top-gc} to Figure \ref{fig:list-alg-full} does not affect its behavior and this change just potentially causes some operations to return sooner, so the same arguments for correctness and time bounds apply (Properties~\ref{space-bound} and~\ref{remove-amortized-time}).
	
	The only remaining changes is that some raw pointers in Figure~\ref{fig:list-alg-full} are replaced with reference counted pointers in Figure~\ref{fig:list-alg-full-gc}.
	As long as a node is not garbage collected while there are still references to them (which was shown in Lemma \ref{lem:step3-safety}), this change does not affect the behavior of the algorithm and thus, it does not affect its correctness.
	In terms of time bounds, \op{tryAppend} performs a constant number of reference counted pointer operations and $R$ \op{remove} operations perform at most $O(R)$ reference counted pointer operations, so the lemma holds.
\end{proof}

\begin{observation}
\label{obs:depreciate-remove}
	\item $M$ calls to \op{vCAS} contains $M$ calls to \op{depreciate} and at most $M$ calls to \op{remove}.
\end{observation}

\begin{definition}
	An \emph{upwards traversal} is when the traversal in the \op{readVersion} operation follows a link from an \lrunreachable{} node to another node. (Note that an upward traversal might move from one node to its descendant.) A \emph{Forward traversal} is when \op{readVersion} follows a link from a \lrreachable{} node to another node. Note that the link is guaranteed to be the a left pointer and that all traversals are either upwards or forwards.
\end{definition}

%\begin{lemma}
%	Suppose node $a$ points to node $b$, then at any earlier configuration in which $a$ is reachable, $b$ is reachable from $a$.
%\end{lemma}
%	
%\begin{proof}
%	
%\end{proof}	

%\begin{lemma}
%\label{lem:list-structure}
%	Given a version list, consider the set of reachable nodes $n_1$, $n_2$, ..., $n_k$ ordered by $\leq_c$.
%	For each $1 \leq i < k$, the following holds:
%	\begin{enumerate}
%		\item $n_i \rightarrow n_{i+1}$, and
%		\item either:
%		\begin{enumerate}
%			\item $n_i \leftarrow n_{i+1}$, or
%			\item $n_{i-1} \leftarrow n_{i+1}$ and $n_{i-1} \leftarrow n_{i}$
%		\end{enumerate}
%	\end{enumerate}
%\end{lemma}
%
%\begin{proof}
%	This is a corollary of Invariant \ref{inv}.
%\end{proof}

\begin{lemma}
\label{lem:traversal}
	Consider the set of upwards traversals in a \op{readVersion} operation.
	The source nodes of these traversals are always distinct.
	Similarly, the destination nodes of forward traversals are always distinct.
	%Let $V$ be a \op{readVersion} operation on object $O$ with timestamp $ts$. Let $ts'$ represent the timestamp in \op{head} after Line \ref{line:readss-initTS-gc} of the \op{readVersion} (this timestamp is guaranteed to be valid). Let $N$ represents the number of \op{vCAS} operations on object $O$ with timestamp between $ts$ (exclusive) and $ts'$ (inclusive). The time complexity of $V$ is $O(N)$ plus the cost of $O(N)$ operations on reference counted pointers.
\end{lemma}

\begin{proof}
	We first prove the first part of the lemma about upwards traversals. Since the left and right pointers of an \lrunreachable{} node always points to nodes that were spliced out later than it (I believe something like this has been proven in step 2), after you perform an upwards traversal leaving $n$, you will never return to $n$. There cannot be a forward traversal to $n$ because otherwise, $n$ would be \lrreachable{}. There cannot be a upwards traversal to $n$ because ... \Hao{need more justification here because there could be a sequence of forward traversals followed by an upwards traversal.} (Note that this statement applies regardless of whether or not the left/right node is an ancestor or a descendant.)
	
	Now we focus on the second part of the lemma about forward traversals.
	Suppose we have a forward traversal $f$ from $Y$ to $Z$.
	Suppose, for contradiction, that at some later configuration, there's another forward traversal $f'$ from $X$ to $Z$ (note that $X$ could possibly be equal to $Y$).
	Consider the path of nodes $\pi = Z, n_1, n_2, ..., n_k, X, Z$ that the traversal visited between $f$ and $f'$.
	We know that $Z$ must have been reachable at all configurations between $f$ and $f'$. \Hao{I assume there's a theorem that says if you become unreachable, you cannot become reachable again.}
	Therefore the transition from $Z$ to $n_1$ must have been a forward traversal.
	By Lemma \ref{order}, we know that $n_1$ has lower counter value than $Z$ because it was a left neighbor of $Z$.
	By the same lemma, we know that $X$ has higher counter value than $Z$.
	Therefore, there are two adjacent nodes, $A$ and $B$, in $\pi$ such that $A$'s counter value is less than or equal to $Z$ and $B$'s counter value is greater.
	Note that $A \neq Z$ because only forward traversals can be performed from $Z$ and these always go left.
	Therefore $A$'s counter value must be less than $Z$.
	Since $\pi$ performs an upwards traversal from $A$ to $B$, $A$ must have been \lrunreachable{} (and therefore finalized) at the time of the traversal and $A \rightarrow B$ so by Invariant \ref{inv}.\ref{no-skip}.\ref{no-skip-right}, all nodes $D$ such that $A \leq_c D \leq_c B$ are unreachable.
	That would imply that $Z$ is unreachable which is a contradiction.
	Therefore, destination nodes of forward traversals are always distinct.

% old proof:
%\begin{itemize}
%	\item Claim: If we perform a forward traversal leaving $n$, then any node that the traversal reaches was reachable from $n$. This is because whenever we perform an upwards traversal, the destination node must have been spliced out after the source node
%	\item Claim: If we perform a forward traversal leaving $n$, then we cannot arrive at a node to the right of $n$ (meaning that it has higher counter value) unless $n$ is spliced out. This is because no node reachable from $n$ via left pointers can point to something to the right of $n$ until $n$ is spliced out (because we first swing left pointers and then swing right pointers).
%	\item Claim: If we perform a forward traversal, the destination node is always unique. Suppose otherwise and there are two forward traversals $A \to C$ and $B \to C$, where $A$ is to the right of $B$. The traversal $B \to C$ must have happened first. Since $C$ is reachable, the next traversal must have been a forward one from $C$ to $D$, but by the previous claim, the traversal cannot return to $A$ until $C$ has been spliced out which is a contradiction.
%\end{itemize}
\end{proof}

\begin{lemma}
\label{lem:up-traversal}
	If \op{readVersion} performs an upwards traversal from $b$ to $c$, then $b$ is a proper ancestor of $c$.
\end{lemma}

\begin{proof}
	If \op{readVersion} performs an upwards traversal from $b$ to $c$, then $b$'s left pointer must be $\top$.
	This means that $b$ must have already been finalized by some \op{splice(a, b, c')} operation.
	We first show that $c = c'$.
	This is because by Property \ref{splice-args} of Invariant \ref{inv}, $b$'s right point must point to $c'$ at the time of the upwards traversal from $b$ to $c$, so $c = c'$.
	To complete the proof, we argue that $c$ is a proper ancestor of $b$.
	Since $b$'s left pointer got set to $\top$, we know that $a \geq_p b$ so by Lemma \ref{splice-priorities}, we know that $b \geq_p c$.
	By lemma \ref{anc-or-desc}, the right neighbor of $b$ is either a proper ancestor or a proper descendant so $c$ is a proper ancestor of $b$.
\end{proof}

\begin{lemma}
\label{lem:common-ancestor}
	Suppose $a$ and $b$ are two nodes in the list such that $a$ is to the left of $b$. Any ancestor of $a$ that is to the right of $b$ is also ancestor of $b$.
\end{lemma}

\begin{proof}
	Let $c$ be an ancestor of $a$ that is to the right of $b$.
	Our goal is to show that $c$ is also an ancestor of $b$.
	We first argue that the least common ancestor (LCA) of $a$ and $b$ is to the left of $b$ and then we argue that $c$ is an ancestor of $LCA(a,b)$. This implies that $c$ is also an ancestor of $b$, as desired.
	We know that $a$ is in the left subtree of $LCA(a,b)$ and $b$ is in the right, so $LCA(a,b)$ must be to the left of $b$.
	This also means that all nodes on the path from $LCA(a,b)$ to $a$ are to the left of $b$.
	Therefore $c$ cannot be on this path, so it must be an ancestor of $LCA(a,b)$, which completes the proof.
\end{proof}

\begin{lemma}
	\label{lem:new-nodes-ancestors}
	If the traversal of a \op{readVersion} operation starts at node $s$, then the nodes visited by the traversal to the right of $s$ must be ancestors of $s$.
\end{lemma}

\begin{proof}
	Let $n_1$, $n_2$, ..., $n_k$ be the set of distinct nodes visited to the right of $s$, sorted in the order in which they were first visited.
	We proceed by induction on this set of nodes.
	Consider the node $n_1$.
	The traversal must have arrived at this node by either leaving $s$ or a node to the left of $s$.
	Call the source node $t$.
	This hop must have been an upwards traversal because it followed $t$'s right pointer so by Lemma \ref{lem:up-traversal}, $n_1$ is an ancestor of $t$.
	By Lemma \ref{lem:common-ancestor}, $n_1$ must also be an ancestor of $s$.
	For the inductive step, suppose $n_i$ is an ancestor of $s$ for all $i < j$.
	It suffices to show that $n_j$ is also an ancestor of $s$.
	There's three ways the traversal could have arrived at this node: (1) from some node $n_i$ where $i < j$, (2) from $s$, or (3) from some node to the left of $s$.
	Cases (2) and (3) are the same as the base case, so we just need to worry about case (1).
	Since an upwards traversal was performed from $n_i$ to $n_j$, by Lemma \ref{lem:up-traversal}, $n_j$ must be an ancestor of $n_i$.
	Since $n_i$ is an ancestor of $s$, $n_j$ is also an ancestor of $s$.
	Therefore, $n_1$, $n_2$, ..., $n_k$ are all ancestors of $s$.
\end{proof}

\begin{lemma}
\label{lem:new-nodes-visited}
	If the traversal of a \op{readVersion} operation starts at node $s$, the number of distinct nodes visited to the right of $s$ is bounded above by both the depth of $s$ in the implicit tree and $O(\log c)$ where $c$ is the number of \op{vCAS} operations concurrent with the \op{readVersion} (on the same object).
\end{lemma}

\begin{proof}
	\Hao{We say that a node is to the right (left) of $s$ if it has higher (lower) counter value.}
	
	Let $n_1, n_2, ..., n_k$ be the $k$ distinct nodes visited by the \op{readVersion} operation to the right of $s$, sorted in order of depth where $n_1$ has the lowest depth.
	By Lemma \ref{lem:new-nodes-ancestors}, each of these $k$ nodes must be an ancestor of $s$, so $k$ is at most the depth of $s$.
	To prove the second part of the Lemma, it suffices show that $c$, the number of \op{vCAS} operations concurrent with the \op{readVersion}, is at least $2^{k-1}$.
	First note that each node $n_i$ was added by a vCAS concurrent with the read-version.
	Next, the subtree rooted at $n_i$ is a complete binary tree which contains all the nodes $n_i, n_{i+1}, ..., n_k$, so its height is at least $k-i+1$. This means that the right subtree of $n_2$ has $2^{k-1}$ nodes and all of these nodes must have been added during the read-version as well (because the entire right subtree of $n_2$ has to be added before $n_1$ is added), which means that $c \geq 2^{k-1}$.
	Therefore, $k \in \min(\log c, \log L)$.
\end{proof}

\begin{theorem}
\label{thm:vcas-gc}
Consider an execution with $R$ calls to \op{vRead}, $T$ calls to the \op{VersionedCAS} constructor (\Hao{maybe we need to account for destructors as well}), $S$ calls to \op{readVersion} and $W$ calls to \op{vCAS}. Suppose the $i$th \op{readVersion} operation is on object $O_i$ with timestamp $ts_i$. 
Let $N_i$ represents the number of successful \op{vCAS} operations on object $O_i$ that (1) were linearized before the start of the \op{readVersion} and (2) have timestamp greather than $ts_i$.
Let $c_i$ represent the number of successful \op{vCAS} operation concurrent with the $i$th \op{readVersion} and let $d_i$ represent the depth (in the implicit tree) of the \vnode{} that the \op{readVersion} started on.
The total time complexity of the \op{VersionedCAS} operations in this execution is $O(R + T + W + \sum_{i=1}^{S} (1+N_i + \min(d_i, \log(c_i+1))))$. \Hao{$N_{vcas}$}
\end{theorem}
\Hao{Say that read version is constant time...}

\begin{proof}
By Observation \ref{obs:depreciate-remove}, the $W$ calls to \op{vCAS} contributes $O(W)$ cost to the total time complexity plus the cost of $O(W)$ calls to \op{C.rt.depreciate} and \op{remove}.
Note that there are no calls to \op{C.rt.depreciate} outside of the \op{vCAS} operation so by Theorem \ref{step1-time}, the total cost of calls to \op{C.rt.depreciate} is $O(W)$.
Similar, the total cost of the $O(W)$ \op{remove} operations is $O(W)$ plus the cost of $O(W)$ operations on reference counted pointers by Lemma \ref{lem:remove-with-gc}.
\Hao{There could also be calls to remove from Figure~\ref{fig:step3-dnode}, which are not accounted for in this argument. These remove operations are only called on the head of a version list so they increase the cost of another remove operation by at most 1.}

Clearly, each call to \op{vRead} and the \op{VersionedCAS} constructor performs a constant number of instructions plus a constant number of reference counted pointer operations.

Next, we will show that the $i$th \op{readVersion} operation performs $O(1 + N_i + \min(d_i, \log(C_i+1)))$ instructions plus (asymptotically) the same amount of reference counted pointer operations.
It suffices to show that the number of distinct nodes visited by the $i$th \op{readVersion} operation is $O(1 + N_i + \min(d_i, \log(c_i+1)))$ because it follows from Lemma \ref{lem:traversal} that the number of upwards and forwards traversals is at most the number of distinct nodes visited.
Each forward and upwards traversal contributes $O(1)$ time plus the cost of $O(1)$ reference counted pointer operations.

By Lemma \ref{lem:new-nodes-visited}, we know that the number of distinct nodes visited to the right of the starting point is at most $O(\min(d_i, \log(c_i+1))$.
Next, we argue that the number of nodes to the left of the starting point is at most $O(1 + N_i)$.
This is because whenever we do a forwards or upwards traversal, we know that the timestamp of the source node is larger than the timestamp of the \op{readVersion} operation.
Thus, all nodes visited to the left of the start node have timestamp greater than $ts$ except one.
Therefore, there are at most $N_i + 1$ such nodes.

Since there are no reference counted pointer operations (affecting Descriptor or VNode objects) outside of Figures~\ref{fig:list-alg-full-gc} and~\ref{fig:vcas-alg-youla-gc} \Hao{this proof doesn't account for the operations from Figure~\ref{fig:step3-dnode}} and since reference counted pointer operations take amortized constant time (Lemma \ref{lem:ref-count} \Hao{We might need to strengthen this lemma}), the total complexity of the \op{VersionedCAS} operations is $O(R + T + W + \sum_{i=1}^{S} (1+N_i + \min(d_i, \log(c_i+1))))$.
\end{proof}

\begin{theorem}
	Snapshot queries take sequential time plus the number of updates concurrent with it. The amortized time of frontier operations remains unchanged.
	\Hao{this theorem needs to be reworded to be more precise. I believe this would be our main result in terms of time complexity.}
\end{theorem}

\Hao{How is \lrreachable{} defined if the head of the version list has been removed?}
\Eric{If it has merely been \co{remove}d then there is no need to define it any differently.
For example, in Lemma \ref{unfinalized-reachable} the proof shows that unfinalized nodes are still
reachable, even after the head node has been \co{remove}d.}
\Hao{I realized my previous question was incorrectly phrased. A more accurate way to say it is "how is lr-reachable defined if the DNode containing the head pointer gets reclaimed"? Under the current definition, all the VNodes in this version list would be unreachable, but some of them might not have been removed yet, and we might want to count them as reachable.}
\Hao{For the heads of the version lists, the space they require is charged to the data structure nodes that point to it. }
%
%
%\begin{lemma} \label{lem:ref-count}
%	If $D$ and $S$ represent the number of deep and shallow external pointers, the number of spliced out \vnode{}s that have a reference counted pointer to it is at most $O(D\log{} L + S + P)$.
%\end{lemma}
%
%\begin{proof}
%	Maybe this should actually say, the number of spliced out nodes with internal pointers to it is at most XYZ.
%	
%	rather than counting deep and shallow pointers, we should probably instead count the number of nodes without internal pointers to them that have not yet been collected.
%	
%	A node can be in 3 states, allocated but not appended, appended but not spliced, spliced but not collected. Internal pointers to a spliced out node can only come from the first and third group. Each process has at most one node in the first group, so there are at most $O(P)$ pointers from such nodes. Nodes in the third group only point to ancestors in the implicit tree except for at most $P$ nodes for which a process paused after splicing the node out and before setting its left/right pointer to $\top$. Therefore there are at most $O(P)$ internal pointers to descendants in the implicit tree.
%	
%	
%	
%	% Maybe first argue for the total number of external pointers, and then argue about the number of deep external pointers.
%\end{proof}

%
%\begin{lemma}
%	There are at most $O(P^2)$ deep external pointers and $O(L_t + P^2)$ shallow external pointers at any configuration.
%\end{lemma}
%
%\begin{theorem}
%
%\end{theorem}

%To prove the bound for $D$ and $S$, we first bound the number of Descriptors. There are at most $2L_t$ that are currently being pointed to by \vnode{}s. This is because spliced out \vnode{}s point to an invalid, frozen Descriptor. All of these $2L_t$ Descriptors contain shallow pointers to \vnode{}s \Hao{need to fill in proof, draw diagram of two cases (perhaps you can cite a lemma from step 2)}. There could be $O(P^2)$ Descriptors that are not pointed to by any \vnode{}s. These include $O(P)$ Descriptors that are held onto only by local pointers, as well as $O(P^2)$ Descriptors that are not pointed to, but are also not yet collected due to deferred decrements. These Descriptors that are not pointed to by any \vnode{} could contain either deep pointers or shallow pointers, so we will conservatively add them to both $D$ and $S$.

%The only other source of external pointers comes from thread local pointers held during vCAS, vRead, readVersion, remove, and tryAppend operations. Again, we will conservatively could these towards both $D$ and $S$. Each thread holds onto a constant number of local pointers so there are at most $O(P)$ of them. Therefore, the number of deep and shallow pointers are bounded by $O(P^2)$ and $O(L_t + P^2)$, respectively.

%There could also be $O(P^2)$ Descriptors that contain deep pointers to \vnode{}s.\Hao{needs to be finished}.

% \Hao{fill in assumption in step 2 about removing the head node.}

%If $L_t$ is the total length of all the version lists, then the number of Descriptors is at most $2L_t + O(P^2)$ because each \vnode{} points to at most 2 Descriptors and $O(P^2)$ could be kept alive due to deferred decrements. \vnode{}s that have been spliced out of their respective version lists do not point to any valid Descriptor objects (their Descriptor fields are finalized before they are removed).
%
%First, we prove the bound on $D$. Each thread holds a constant number of local pointers, which contributions at most $O(P)$ to the number of deep external pointers. There could also be $O(P^2)$ deep external pointers from the $O(P^2)$ Descriptors
%
%, so these contribute $O(P)$ to the total.
%
%To bound the number of Descriptors, we note that there are only two types of pointers to these objects. A Descriptor can be pointed to by at most one \vnode{} and possibly multiple thread local pointers. There are at most a constant number of local pointers per thread, and each \vnode{} in the version list points to at most two Descriptors, so the number of Descriptors being pointed to is at most two times the total length of the version lists (plus $O(P)$). Note that all spliced out \vnode{} point to the invalid (frozen) Descriptor. Due to deferred decrements, there could also be $O(P^2)$ Descriptors that do not have any pointers to them and are not yet collected.
%
%In terms of time bounds, using the algorithm from~\cite{}, all operations on \rcptr{}s and \arcptr{}s take constant time, so

%\Hao{talk about overall space bounds.}
%\Hao{perhaps "spliced out nodes" should just be called "unreachable nodes".}
%\Hao{talk about the syntax for rc pointers. rc pointers can be compared with each other as well as null pointers. rc pointers need to support non-pointer values. I guess the non-pointer values can just be dummy objects.}
%\Hao{I'm not sure if I should be using rc pointer syntax as it requires some understanding of C++.}

%\begin{itemize}
%	\item The only tricky part is proving that the Descriptors do not prevent the collection of too many nodes. This is the case because because as long as A's right Descriptor points to A, B and C, the list is either in the state (A <- B -> C and A <-> C) or (A <-> B <-> C). In either case, these references do not prevent the collection of a huge chain of nodes. Then we just need to argue that the $P^2$ delayed decrements do not hold onto too many nodes.
%	\item note that unreachable nodes do not point to Descriptors
%	\item traversal algorithm, keep traversing left until you hit a node whose left pointer is null, then traverse right. It's guaranteed that you won't visit that node again because it has already been completely spliced out, so once you start traversing left again, you'll skip over it. \Hao{double check this} Therefore all right traversals from node A to node B have distinct A values. We just need to say something like this about left traversals. I think they have distinct B values. Suppose you move left twice, once from A to B and once from A' to B', I think we can show that B' has strictly smaller counter value compared to B. This is clearly true if the two are consecutive (B == A'). Otherwise, there's a sequence of right traversals from B to A', then the nodes in the range [B, A) were spliced out before A'. If A' is not spliced out, then A' will skip past these nodes. If A' was spliced out, ... \Hao{TODO: complete proof}
%\end{itemize}

\Hao{make remove-rec camel case.}

\begin{figure*}[!th]\small
	%\vspace{-.1in}
	\begin{minipage}[t]{.47\textwidth}
		\begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none]
class Camera {
	int timestamp;
	RangeTracker<VNode*> rt;
	Camera() { timestamp = 0; }   @\label{line:ss-con}@
	
	int takeSnapshot() {
		int ts = rt.Announce(timestamp, pid); @\label{line:read-time}@
		CAS(&timestamp, ts, ts+1);    @\label{line:inc-time}@
		return ts; }
	
	void unreserve() {
		rt.@\Unannounce@(pid); } };
	
	class VNode {
		Value val; arc_ptr<VNode> left, right; int ts;
		// the remaining variables are only
		// used by remove() and tryAppend()
		int priority; int counter;
		enum status; int refCount;
		VNode(Value v) {
			val = v; ts = TBD; } };
	
	class VersionedCAS {
		VersionList VList;
		Camera* C;
		VersionedCAS(Value v, Camera* c) {           @\label{line:vcas-con}@
			C = c;
			rc_ptr<VNode> node = new VNode(v);
			VList.tryAppend(null, node);
			initTS(node);		
				\end{lstlisting}
			\end{minipage}\hspace{.3in}
			\begin{minipage}[t]{.49\textwidth}%xleftmargin=5.0ex,
				\StartLineAt{32}
				\begin{lstlisting}[linewidth=.99\textwidth, numbers=left, frame=none]
void initTS(rc_ptr<VNode> n) {
	if(n->ts == TBD) {               @\label{line:init1-gc}@
		int curTS = C->timestamp;       @\label{line:readTS-gc}@
		CAS(&(n->ts), TBD, curTS); } }   @\label{line:casTS-gc}@

Value readVersion(int ts) {
	rc_ptr<VNode> node = VList.getHead();     @\label{line:readss-head-gc}@
	initTS(node);                     @\label{line:readss-initTS-gc}@
	node = VList.find(node, ts);
	return node->val; } // node cannot be null       @\label{line:readss-ret-gc}@

Value vRead() {
	rc_ptr<VNode> head = VList.getHead();         @\label{line:readHead-gc}@
	initTS(head);                         @\label{line:read-initTS-gc}@
	return head->val; }

bool vCAS(Value oldV, Value newV) {
	rc_ptr<VNode> head = VList.getHead();         @\label{line:vcas-head-gc}@
	initTS(head);                         @\label{line:vcas-initTS-gc}@
	if(head->val != oldV) return false;   @\label{line:vcas-false1-gc}@
	if(newV == oldV) return true;         @\label{line:vcas-true1-gc}@
	rc_ptr<VNode> newN = new VNode(newV);        @\label{line:newnode-gc}@
	if(VList.tryAppend(head, newN)) {        @\label{line:append-gc}@
		initTS(newN);                       @\label{line:initTSnewN-gc}@
		List<VNode*> redundant = C.rt.@\retireInterval @(
		@\hil{head.getPtr()}@, head.ts, newN.ts);
		forevery(node in redundant) {
			@\hil{// convert from raw pointer to}@
			@\hil{// reference counted pointer}@
			@\hil{rc\_ptr<VNode> rc\_node = node;}@ @\label{line:to-rc-ptr}@
			remove(rc_node); }
		return true; }                      @\label{line:vcas-true2-gc}@
	else {
		delete newN;                        @\label{line:scdelete-gc}@
		initTS(VList.getHead());                      @\label{line:vcas-initTSHead-gc}@
		return false; } } };                   @\label{line:vcas-false2-gc}@

class VersionList {
	// Includes the remove() and tryAppend() methods as well
	arc_ptr<VNode> Head;
	
	rc_ptr<VNode> getHead() {
	 	return Head.load(); }
	
	// precondition: node != null
	// precondition: some tryAppend(*, start) linearized
	// Need to argue that if a node's left pointer is top, then its right pointer has been initialized. This is because a node's right pointer is initialized before remove can be called on it.
	rc_ptr<VNode> find(rc_ptr<VNode> start, int ts) {
	 	rc_ptr<VNode> current = start;
	 	while(current->ts > ts) {
	 		@\hil{rc\_ptr<VNode> next = current->left;}@
	 		@\hil{if(next == $\top$) next = current->right;}@
	 		@\hil{current = next;}@ }
	 	return current; } };
			\end{lstlisting}
		\end{minipage}
		\vspace{-.1in}
		\caption{Indirect \vCAS{} implementation using the previously defined interval tracker and version list interface.
		\Eric{Just give new versions of readVersion and mention in text the conversion between raw pointers and reference counted pointers at line \ref{line:to-rc-ptr}.  Is it even necessary to say head.getPtr(), since we say in text that \rcptr\ supports standard ops that raw pointers support?}
		\Eric{Right now, this figure is causing problems with multiply-defined labels}
		}
		\label{fig:vcas-alg-youla-gc}
		%\vspace{-1in}
	\end{figure*}

\begin{figure*}[!th]\small
	%\vspace{-.1in}
	\begin{minipage}[t]{.47\textwidth}
		\begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none]
global variables:			
RangeTracker<DNode*> dnodeTracker;
// this range tracker should share an announcement
// array with the range tracker for vnodes

void setBirthTS(DNode* node) {
	// We have to know which Camera object (C)
	// node belongs to somehow. Maybe we should
	// just make the Camera object global.
	node->birthTS = C.timestamp; }

void setRetireTS(DNode* node) {
	node->reitreTS = C.timestamp; }
		\end{lstlisting}
	\end{minipage}\hspace{.3in}
	\begin{minipage}[t]{.47\textwidth}%xleftmargin=5.0ex,
		\StartLineAt{29}
		\begin{lstlisting}[linewidth=.99\textwidth, numbers=left, frame=none]
void freeDNode(DNode* node) {
	List<DNode*> removable =
	dnodeTracker.retireInterval(
	node, node->birthTS, node->retireTS);
	for(dnode in removable) {
		// the following should maybe go in
		// VersionedCAS's destructor
		for each VersionedCAS field (F) of dnode {
			remove(dnode.F.VHead); }
		free(dnode); } }
	\end{lstlisting}
\end{minipage}
\vspace{-.1in}
\caption{Step 3: code for reclaiming \dnode{}s. \Hao{The description in the text is clear enough that we can get rid of this pseudo-code. I'm leaving it here for now because it is a concise summary of how the algorithm works.}}
\label{fig:step3-dnode}
\end{figure*}

%rough notes:
%- This step might not be as hard as I initially thought
%- 2 level GC: The frontier operations and the snapshot queries use different GC techniques. A node can only be freed once it is freed by both. Our paper only focuses on snapshot operation GC.
%- You can either use HP for frontier operations or EBR for frontier operations and our MVGC technique only for snapshot operations. This approach works for direct vCAS objects too.
%- This technique will add time overhead but it's low memory overhead is useful in memory constrained environments or snapshots that will be kept around for a long time (for example for debugging, check pointing, time travel queries, or interactive user queries. This can also be used for example to take one snapshot every day and maintain snapshots for the past 5 days. Maybe look at how snapshotting is used in RockDB).
%- Realistic workloads: What kind of update frequency would you expect in a realistic workload? In our experiments, we have 36 constantly performing updates (which is why EBR uses up so much space), but that's probably never happens in practice. 

==> version-list-alg-direct.tex <==
% !TEX root =  main.tex

\section{Removing from a Version List (direct vCAS)}

\begin{figure*}[!th]\small
	%\vspace{-.1in}
	\begin{minipage}[t]{.49\textwidth}
		\begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none, language=C++, morekeywords=class]
class List<Node extends ListNode> {
	Node* Head;

	List(ListNode* X) { Head = X; } 
	Node* getHead() { return Head; }
	
	bool tryAppend(Node* old, Node* new) {
		return tryAppend(old, new); }
	
	Node* find(Predicate P) {
		Node* node = Head;
		while(node != null and !P(node)) {
			node = readLeft(node); }
		return node; }
	
	void remove(Node* Y) {
		setMark(Y);
		remove-rec(Y); }
			\end{lstlisting}
		\end{minipage}\hspace{.3in}
		\begin{minipage}[t]{.49\textwidth}%xleftmargin=5.0ex,
			\StartLineAt{20}
			\begin{lstlisting}[linewidth=.99\textwidth, numbers=left, frame=none]
	// x,y,z denotes the numbers
	// stored in X,Y,Z respectively
	// unless otherwise noted
	void remove-rec(Node* Y) {
		Node* X = readLeft(Y);
		if(X == null) x = INF;
		Node* Z = readRight(Y);
		bool recurse = false;
		if(x > y < z) recurse = splice(X, Y, Z)
		else if(x < y < z)
		recurse = spliceUnmarkedLeft(X, Y, Z)
		else if(x > y > z)
		recurse = spliceUnmarkedRight(X, Y, Z)
		if(recurse) {
			If X is null, call remove-rec() on Z.
			Else if only one of {X, Z} is marked,
			then call remove-rec() on whichever
			one is marked.
			Else if both are marked, call
			remove-rec() on whichever one has
			smaller number. } } };
		\end{lstlisting}
	\end{minipage}
	\vspace{-.1in}
	\caption{Linearizable implementation of the list data structure. This implementation is for direct vCAS objects. [TODO: use different font for publicly exposed methods.]}
	\label{fig:vcas-alg}
	%\vspace{-1in}
\end{figure*}

\begin{figure*}[!th]\small
	%\vspace{-.1in}
	\begin{minipage}[t]{.49\textwidth}
		\begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none, language=C++, morekeywords=class]			
			class Node {
				Node* left, right; // initially null
				enum status; // initially unmarked
				int num; // defines implicit tree
				Descriptor* leftDesc;  // initially null
				Descriptor* rightDesc; // initially null
			};
			
			class Descriptor { Node* X, Y, Z; };
			Descriptor* fin = new Descriptor();
			
			bool tryAppend(Node* old, Node* new) {
				return tryAppend(old, new);
				if(head != old) return false;
				setLeft(new, old);
				// help set right pointer
				// This wouldn't work for indirect vcas
				Node* n = getLeft(old);
				if(n != null) casRight(n, null, old);
				if(CAS(&head, old, new)) {
					casRight(old, null, new); 
					return true; }
				else return false; }
			
			// splice has to work even when X is null
			// I believe we do not have to update 
			// spliceUnmarkedRight
			bool splice(Node* X, Node* Y, Node* Z) {
				// help Z->left
				Node* A = Z->left;
				if(A->left = Y) CAS(&(Z->left), A, Y);
				// help X->right if X is not null
				if(X != null) {
					Node* A = X->right;
					if(A->right = Y) CAS(&(X->right), A, Y); }
				if(!CAS(&(Y->status), marking, finalized)) 
				return false;
				if(X != null) CAS(&(X->right), Y, Z);
				CAS(&(Z->left), Y, X);
				return true; }
			
			Node* readRight(Node* X) {
				Node* Y = X->right;
				if(Y->status == finalized) {
					Node* Z = Y->right;
					CAS(&(X->right), Y, Z); 
					return Z; }
				else return Y; }
			
			Node* readLeft(Node* Z) {
				Node* Y = Z->left;
				if(Y->status == finalized) {
					Node* X = Y->left;
					CAS(&(Z->left), Y, X); 
					return X; }
				else return Y; }
		\end{lstlisting}
	\end{minipage}\hspace{.3in}
	\begin{minipage}[t]{.49\textwidth}%xleftmargin=5.0ex,
		\StartLineAt{40}
		\begin{lstlisting}[linewidth=.99\textwidth, numbers=left, frame=none]
			void setMark(Node* X) {
				X->status = marking;
				helpSetMark(X); }
			
			void isMarked(Node* X) {
				if(X->status == unmarked) return false;
				if(X->status == finalized) return true;
				if(X->status == marking) {
					helpSetMark(X);
					return true; } }
			
			void helpSetMark(Node* X) {
				for F in [leftDesc, rightDesc] {
					repeat twice {
						Descriptor* desc = X->F;
						help(desc);
						CAS(&(X->F), desc, fin); } } }
			
			// X is guaranteed to not be null
			bool spliceUnmarkedLeft(Node* X, Node* Y, Node* Z) {
				Descriptor* oldDesc = X->rightDesc;
				if(X->status == marking) {
					helpSetMark(X);
					return false; }
				else if(X->status == finalized)
				return false;
				if(X->right != Y) return false;
				help(oldDesc); // this help might not be necessary 
				Descriptor* newDesc = new Descriptor(X, Y, Z);
				bool succ = CAS(&(X->rightDesc), oldDesc, newDesc);
				if(X->rightDesc = fin) {
					helpSetMark(X);
					return false; }
				help(X->rightDesc);
				return succ; }
			
			void help(Descriptor* desc) {
				if(desc != null && desc != fin)
				splice(desc->X, desc->Y, desc->Z); }
		\end{lstlisting}
	\end{minipage}
	\vspace{-.1in}
	\caption{Linearizable implementation of helper functions. This implementation is for direct vCAS objects.}
	\label{fig:vcas-alg}
	%\vspace{-1in}
\end{figure*}


==> version-list-alg-youla.tex <==
% !TEX root =  main.tex

%Potentially useful properties: Left and right pointers are ABA-free meaning that they will never point to the same node twice. The only "conflicts" are between setMark and spliceUnmarkedLeft (or spliceUnmarkedRight). 

\section{Version List Algorithm (Youla)}

The \op{Remove} algorithm uses 7 helper functions, \op{readLeft}, \op{readRight}, \op{setMark}, \op{isMarked}, \op{splice}, \op{spliceUnmarkedLeft} and \op{spliceUnmarkedRight}, which are all linearizable. 
These 7 operations should ideally take constant time.
The sequential specifications of some of these helper functions is described below:

\begin{itemize}
	\item \op{splice(W, X, Y)}: if W and Y are left and right (respectively) neighbors of X, then splice out X and return true. Otherwise, return false.
	\item \op{spliceUnmarkedLeft(W, X, Y)}: if \op{W} and \op{Y} are left and right (respectively) neighbors of \op{X}, and \op{W} is unmarked then splice out \op{X} and return true. Otherwise, return false.
	\item \op{spliceUnmarkedRight(W, X, Y)}: Similar to \op{spliceUnmarkedLeft(W, X, Y)} except \op{Y} has to be unmarked.
\end{itemize}


To implement the 7 helper functions, we add a status field to each node which can either be \op{unmarked}, \op{marked}, or \op{finalized}.
Each node starts off being \op{unmarked}, and later transitions to being \op{marked} at the beginning of a \op{setMark} operation (this is not where the \op{setMark} is linearized).
One of the three splice operations will later set a node's status to be \op{finalized}.
A splice operation is linearized when it sets a node's status to \op{finalized}.
When a \op{readLeft} or \op{readRight} comes across a finalized node, it has to help splice out that node.
An important property is that there cannot be two finalized nodes in a row.

To implement these helper functions, we also add two more fields: \op{rightDesc} and \op{leftDesc}. These fields point to descriptor objects and are initially null. They are used by \op{spliceUnmarkedLeft} and \op{spliceUnmarkedRight} to prevent a node from being marked while a splice is in progress.
The \op{setMark} operation sets both \op{rightDesc} and \op{leftDesc} to \op{fin} to prevent any more descriptors from being installed on the node, and it is linearized when both descriptors have been set to \op{fin}.

\begin{figure*}[!th]\small
%\vspace{-.1in}
\begin{minipage}[t]{.49\textwidth}
  \begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none]
// Worst-case time: O(log L) 
// where L is measured at the
// start of the operation
// Amortized time: O(1)

class Node {
  Node* left, right; // initially null
  enum status; // initially unmarked
  int num; // defines implicit tree
};

void remove(Node* X) {
  X->status = marked;
  remove-rec(X); }

// w,x,y denotes the numbers
// stored in W,X,Y respectively
void remove-rec(Node* X) {
  Node* W = X->left;
  Node* Y = X->right;
  bool recurse = false;
  if(w > x < y) recurse = splice(W, X, Y) @\label{test-priority} \label{call-splice}@ 
  if(recurse) {
    if only one of {W, Y} is marked,
    then call remove-rec() on whichever
    one is marked.
    If both are marked, then call
    remove-rec() on whichever one has
    smaller number. 
  } 
}


bool splice(Node* W, Node* X, Node* Y) {
	if (!CAS(&(X->status), marked, finalized)) @\label{finalize-cas}@
	    return false; 
  if (w>y) {                   @\label{priority-switch}@
      CAS(&(W->right), X, Y);  @\label{right-cas1}@
      CAS(&(Y->left), X, W);   @\label{left-cas1}@
  }
  else {
      CAS(&(Y->left), X, W);   @\label{left-cas2}@
      CAS(&(W->right), X, Y);  @\label{right-cas2}@
  }
  return true; }
  \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{.49\textwidth}
	\begin{lstlisting}[linewidth=.99\columnwidth, numbers=left,frame=none]
// Y is a newly appended node whose left pointer
// points to X.
// This method sets X's right pointer to Y
// and initializes the number and status
// in Y.
void makeRemovable(Node* X, Node* Y) {
	Y.counter = X.counter+1;
	Y.num = lowestSetBit(Y.counter);
	CAS(&(X.right), null, Y);
}
  \end{lstlisting}
\end{minipage}
\vspace{-.1in}
  \caption{Linearizable implementation of \label{break-ties}
  }
\label{fig:vcas-alg-simplified}
%\vspace{-1in}
\end{figure*}




==> version-list-alg.tex <==
% !TEX root =  main.tex

\section{Removing from a Version List}

%Potentially useful properties: Left and right pointers are ABA-free meaning that they will never point to the same node twice. The only "conflicts" are between setMark and spliceUnmarkedLeft (or spliceUnmarkedRight). 

\subsection{Helper Functions}

The \op{Remove} algorithm uses 7 helper functions, \op{readLeft}, \op{readRight}, \op{setMark}, \op{isMarked}, \op{splice}, \op{spliceUnmarkedLeft} and \op{spliceUnmarkedRight}, which are all linearizable.
These 7 operations should ideally take constant time.
The sequential specifications of some of these helper functions is described below:

\begin{itemize}
	\item \op{splice(W, X, Y)}: if W and Y are left and right (respectively) neighbors of X, then splice out X and return true. Otherwise, return false.
	\item \op{spliceUnmarkedLeft(W, X, Y)}: if \op{W} and \op{Y} are left and right (respectively) neighbors of \op{X}, and \op{W} is unmarked then splice out \op{X} and return true. Otherwise, return false.
	\item \op{spliceUnmarkedRight(W, X, Y)}: Similar to \op{spliceUnmarkedLeft(W, X, Y)} except \op{Y} has to be unmarked.
\end{itemize}

To implement the 7 helper functions, we add a status field to each node which can either be \op{unmarked}, \op{marking}, or \op{finalized}.
Each node starts off being \op{unmarked}, and later transitions to being \op{marking} at the beginning of a \op{setMark} operation (this is not where the \op{setMark} is linearized).
One of the three splice operations will later set a node's status to be \op{finalized}.
A splice operation is linearized when it sets a node's status to \op{finalized}.
When a \op{readLeft} or \op{readRight} comes across a finalized node, it has to help splice out that node.
An important property is that there cannot be two finalized nodes in a row.

To implement these helper functions, we also add two more fields: \op{rightDesc} and \op{leftDesc}. These fields point to descriptor objects and are initially null. They are used by \op{spliceUnmarkedLeft} and \op{spliceUnmarkedRight} to prevent a node from being marked while a splice is in progress.
The \op{setMark} operation sets both \op{rightDesc} and \op{leftDesc} to \op{fin} to prevent any more descriptors from being installed on the node, and it is linearized when both descriptors have been set to \op{fin}.

% TODO: change remove() to work for tail nodes.


